Fuzzy Logic Based Logical Query Answering on Knowledge Graphs

Answering complex First-Order Logical (FOL) queries on large-scale incomplete knowledge graphs (KGs) is an important yet challenging task. Recent advances embed logical queries and KG entities in the same space and conduct query answering via dense similarity search. However, most logical operators designed in previous studies do not satisfy the axiomatic system of classical logic, limiting their performance. Moreover, these logical operators are parameterized and thus require many complex FOL queries as training data, which are often arduous to collect or even inaccessible in most real-world KGs. We thus present FuzzQE, a fuzzy logic based logical query embedding framework for answering FOL queries over KGs. FuzzQE follows fuzzy logic to define logical operators in a principled and learning-free manner, where only entity and relation embeddings require learning. FuzzQE can further benefit from labeled complex logical queries for training. Extensive experiments on two benchmark datasets demonstrate that FuzzQE provides significantly better performance in answering FOL queries compared to state-of-the-art methods. In addition, FuzzQE trained with only KG link prediction can achieve comparable performance to those trained with extra complex query data.

==> tables/axioms.tex <==
\begin{table}[t]
\footnotesize
\centering
\caption{Here we list some axioms
% written in Hilbert-style deductive system 
that are shared by classical logic and fuzzy logic and give the corresponding properties that a query embedding model should possess. 
The axiomatic systems and analysis are provided in Appendix \ref{ap:axioms}. 
$\varphi, \psi, \chi$ represent logical formulae.
$\phi$ denotes the scoring function that
estimates the probability that the entity $q$ can answer the query $q$. 
}
\begin{tabular}{lll}
\toprule
     & Axioms & Model Property \\
\midrule
% $\rightarrow$
%     &
%     & $\phi(q, e) \geq \phi(q,e')$, if KB implies q[e],
%     % $\phi(q,e') < 1$, 
%     if KB does not implies q[e']
%     \\

\multirow{5}{*}{$\land$} 
    & $\varphi \wedge \psi \rightarrow \varphi$
    & $\phi(q_1 \land q_2, e) \leq \phi(q_1, e) $ \\
    \cmidrule(lr){2-3}
    
    & $\varphi \wedge \psi \rightarrow \psi$
    & $\phi(q_1 \land q_2, e) \leq \phi(q_2, e) $ \\
    \cmidrule(lr){2-3}
    
    & $(\chi \rightarrow \varphi) \rightarrow$
        & $\phi((q_1 \land q_2), e) = \phi((q_2 \land q_1), e)  $ \\
        \cmidrule(lr){3-3}
    & $((\chi \rightarrow \psi) \rightarrow$
        & $\phi((q_1 \land q_2) \land q_3, e) $ \\
    & $(\chi \rightarrow \varphi \wedge \psi))$
        & $= \phi(q_1 \land (q_2 \land q_3), e)$ \\
\midrule

\multirow{5}{*}{$\lor$} 
    & $\varphi \rightarrow \varphi \vee \psi$
    & $\phi(q_1 \lor q_2, e) \geq \phi(q_1, e) $ \\
    \cmidrule(lr){2-3}
    
    & $\varphi \rightarrow \varphi \vee \varphi$
    & $\phi(q_1 \lor q_2, e) \geq \phi(q_2, e) $ \\
    \cmidrule(lr){2-3}

    & $(\chi \rightarrow \varphi) \rightarrow$
        & $\phi((q_1 \lor q_2), e) = \phi((q_2 \lor q_1), e)  $  \\
        \cmidrule(lr){3-3}
    & $((\chi \rightarrow \psi) \rightarrow$
        & $\phi((q_1 \lor q_2) \lor q_3, e)  $ \\
    & $(\chi \rightarrow \varphi \lor \psi))$
        & $ = \phi(q_1 \lor (q_2 \lor q_3), e)$\\
\midrule

$\neg$
    & $\neg \neg \varphi \rightarrow \varphi$ 
        & $\phi(q, e) = \phi(\neg \neg q, e)$ \\
    \cmidrule(lr){2-3}
    
    
    & $\varphi \land \neg \varphi \rightarrow \overline{0}$
        & $\phi(q, e) \uparrow \quad \Rightarrow \quad \phi(\neg q, e) \downarrow $\\
\bottomrule  
\end{tabular}
\label{tab:axioms}
\end{table}

==> tables/baseline-geo.tex <==
\begin{table*}[h]
    \footnotesize
    \centering
    \caption{A comparison of how entities and queries are embedded in different models and how logical operators are implemented.
    Min denotes element-wise minimum.
    CEN, OFF for Query2Box represents the center vector and the offset vector of the box respectively.
    $\gamma$ for Query2Box is a deep architecture based coefficient to shrink the result box size.
    % \emph{Beta.} stands for Beta distribution, and 
    $\mathcal{B}[\alpha, \beta]$ denotes the beta distribution with parameter $\alpha$ and $\beta$.
    \emph{DNF} means that the model first rewrites the query to Disjunctive Normal Form (DNF) and then retains all input embeddings at the last step.
    \emph{DM} stands for De Morgan's law.
    [FuzzQE interpretation needs update]
    %//TODO: fill up FuzzQE entity, query interpretation
    %//TODO: distance update as \phi
    }
    \label{table:baseline-geo}
    \begin{tabular}{lllllll}
    \toprule
        & Entity $e$ 
        & Query $q$ 
        & $q_1 \land q_2$  
        & $q_1 \lor q_2$ 
        & $\neg q$ 
        & Metric  \\
    \midrule

    \multirow{2}{*}{GQE}    
        &  point 
        &  point 
        &  mean
        &  \multirow{2}{*}{DNF}
        &  \multirow{2}{*}{N/A}  
        & \multirow{2}{*}{cos}               
    \\
        &  $\be \in \mathbb{R}^d$ 
        &  $\bsq \in \mathbb{R}^d$ 
        & $\frac{1}{2} (\bsq_1 + \bsq_2)$
        &  
        &   
        &  
    \\   
    \midrule

    \multirow{3}{*}{Query2Box}    
        &  point 
        &  box 
        & box intersection 
        &  \multirow{3}{*}{DNF}
        &  \multirow{3}{*}{N/A}  
        & point-to-box          
    \\
        &  $\be \in \mathbb{R}^d$ 
        &  $\text{CEN}_q \in \mathbb{R}^{d}$ 
        &  $\frac{1}{2} (\text{CEN}_{q_1} + \text{CEN}_{q_2})$ 
        &  
        &   
        &  distance
    \\   
        & 
        &  $\text{OFF}_q \in \mathbb{R}^{d}$ 
        &  $\gamma \text{Min} (\text{OFF}_{q_1}, \text{OFF}_{q_2})$ 
        &  
        &   
        & 
    \\   
    \midrule

    \multirow{2}{*}{BetaE}   
        % //TODO: update to q_alpha, q_beta
        % make the formula double rows
        &  \multirow{2}{*}{$\mathcal{B}[\alpha_e, \beta_e]$}
        &  \multirow{2}{*}{$\mathcal{B}[\alpha_q, \beta_q]$}
        &  \multirow{2}{*}{$\mathcal{B}[\frac{1}{2}(\alpha_{q_1}+\alpha_{q_2}), 
        \frac{1}{2}(\beta{q_1}+\beta{q_2})]$}
        &  (i) DNF 
        & \multirow{2}{*}{$\mathcal{B}[1/\alpha_q, 1/\beta_q]$} 
        & \multirow{2}{*}{KL divergence}  
    \\
    % \cmidrule(lr){5-5}
        & 
        & 
        & 
        & (ii) DM
        &                                       
        &    
    \\

    % \midrule
    % %% our model
    % \multirow{2}{*}{$\modelname$}   
    %     & entity                   
    %     & query                      
    %     &  fuzzy conjunction 
    %     &  fuzzy disjunction
    %     &  fuzzy negation 
    %     &  \multirow{2}{*}{dot product}     
    % \\
    %     & $\be \in [0,1]^d$
    %     & $\bsq \in [0,1]^d$
    %     & $\bsq_1 \circ \bsq_2$
    %     & $\bsq_1 + \bsq_2 - \bsq_1 \circ \bsq_2$
    %     & $\mathbf{1} - \bsq$
    %     &
    % \\


    % \midrule
    % %% our model
    % \multirow{2}{*}{$\modelname$}   
    %     & \multirow{2}{*}{entity}                    
    %     & \multirow{2}{*}{query}                      
    %     &  fuzzy conjunction 
    %     &  fuzzy disjunction
    %     &  fuzzy negation 
    %     &  \multirow{2}{*}{dot product}     
    % \\
    %     &
    %     &
    %     & (t-norm) 
    %     & (t-conorm) 
    %     & (Lukasiewicz negator) 
    %     &
    % \\


    \bottomrule
    \end{tabular}
\end{table*}
    

==> tables/logiclaws-copy.tex <==
\begin{table*}[t]
    \small
    \centering
    \begin{tabular}{ll|l|l}
    \toprule
         & \multicolumn{2}{c}{Logic Law} & Model Property \\
    \midrule
    % $\rightarrow$
    %     &
    %     & $\phi(q, e) \geq \phi(q,e')$, if KB implies q[e],
    %     % $\phi(q,e') < 1$, 
    %     if KB does not implies q[e']
    %     \\
    \multirow{9}{*}{$\land$} 
        & & Conjunction  & \\
        & & Elimination & \\
        & \multirow{2}{*}{\myroman{1}} & $\psi_1 \wedge \psi_2 \rightarrow \psi_1$
        & $\phi(q_1 \land q_2, e) \leq \phi(q_1, e) $ \\
        % \cmidrule(lr){2-3}
        
        & & $\psi_1 \wedge \psi_2 \rightarrow \psi_2$
        & $\phi(q_1 \land q_2, e) \leq \phi(q_2, e) $ \\
        \cmidrule(lr){2-4}
        
        & & Commutativity & \\
        & \myroman{2} & $\psi_1 \land \psi_2 \leftrightarrow \psi_2 \land \psi_1$
            & $\phi((q_1 \land q_2), e) = \phi((q_2 \land q_1), e)  $ \\
        \cmidrule(lr){2-4}
        
        & &  Associativity & \\
        & \myroman{3} & $(\psi_1 \land \psi_2) \land \psi_3 \leftrightarrow$
            & $\phi((q_1 \land q_2) \land q_3, e) $ \\
        & & $\psi_1 \land (\psi_2 \land \psi_3)$
            & $= \phi(q_1 \land (q_2 \land q_3), e)$ \\
    \midrule
    
    \multirow{9}{*}{$\lor$} 
        & & Disjunction  & \\
        & & Amplification & \\
        & \multirow{2}{*}{\myroman{4}} & $\psi_1 \rightarrow \psi_1 \vee \psi_2$
        & $\phi(q_1, e) \leq \phi(q_1 \lor q_2, e) $ \\
        % \cmidrule(lr){2-3}
        
        & & $\psi_2 \rightarrow \psi_1 \vee \psi_2$
        & $\phi(q_2, e) \leq \phi(q_1 \lor q_2, e) $ \\
        \cmidrule(lr){2-4}
    
        & & Commutativity & \\
        & \myroman{5} & $\psi_1 \lor \psi_2 \leftrightarrow \psi_2 \lor \psi_1$
            & $\phi((q_1 \lor q_2), e) = \phi((q_2 \lor q_1), e)  $  \\
        \cmidrule(lr){2-4}
        & & Associativity & \\
        & \myroman{6} & $(\psi_1 \lor \psi_2) \lor \psi_3 \leftrightarrow$
            & $\phi((q_1 \lor q_2) \lor q_3, e)  $ \\
        & & $\psi_1 \lor (\psi_2 \lor \psi_3)$
            & $ = \phi(q_1 \lor (q_2 \lor q_3), e)$\\
    \midrule
    
    \multirow{4}{*}{$\neg$} 
        & & Involution & \\
        & \myroman{7} & $\neg \neg \psi_1 \rightarrow \psi_1$ 
            & $\phi(q, e) = \phi(\neg \neg q, e)$ \\
        \cmidrule(lr){2-4}
        
        & & Non-Contradiction & \\
        & \myroman{8} & $\psi_1 \land \neg \psi_1 \rightarrow \overline{0}$
            & $\phi(q, e) \uparrow \quad \Rightarrow \quad \phi(\neg q, e) \downarrow $\\
    \bottomrule  
    \end{tabular}
    \caption{
    % \YS{which text cites this table?} \shirley{It is cited in Section 3.1.} 
    Here we list eight logic laws (I - VIII) 
    % written in Hilbert-style deductive system 
    from classical logic 
    % and fuzzy logic axiomatic systems
    \cite{fuzzytheorybook} and give the corresponding properties that a query embedding model should possess.
    %They are based on the Modus Ponen inference rule ``$\text{from}~\psi_1~\text{and}~\psi_1 \rightarrow \psi_2
    %~\text{infer}~\psi_2$'' and the implication semantics ``$\psi_1 \rightarrow \psi_2$ holds if the truth value of $\psi_2$ is larger than or equal to $\psi_1$''.
    $\psi_1, \psi_2, \psi_3$ represent logical formulae.
    $\phi$ denotes the scoring function that
    estimates the probability that the entity $e$ can answer the query $q$. 
    $\phi(q, e) \uparrow \Rightarrow \phi(\neg q, e) \downarrow $ means $\phi(\neg q, e)$ is monotonically decreasing with regard to $\phi(q, e)$. The full axiomatic systems and analysis are provided in Appendix \ref{ap:axioms}. 
    % \YS{I changed the labelling. Please be consistent in Table 6.}
    % \YS{do we really need greek letters if we already have $q_1,q_2$? How about using $q_1$ to denote the logical expression of $q_1$ and use $\mathbf{q}_1$ to denote its embedding, which is used in score function $\phi$?}
    % \shirley{I think it might be better to present the fundamental logic laws without regard to the task. Using $q$ for logic laws may look task-specific.}
    }
    %//TODO: update Table 6 to make notation consistent
    \label{tab:axioms}
    \end{table*}
    
    
    
    % \multirow{9}{*}{$\land$} 
    %     & & Conjunction  & \\
    %     & & Elimination & \\
    %     & \multirow{2}{*}{\myroman{1}} & $\psi_1 \wedge \psi_2 \rightarrow \psi_1$
    %     & $\phi(q_1 \land q_2, e) \leq \phi(q_1, e) $ \\
    %     % \cmidrule(lr){2-3}
        
    %     & & $\psi_1 \wedge \psi_2 \rightarrow \psi_2$
    %     & $\phi(q_1 \land q_2, e) \leq \phi(q_2, e) $ \\
    %     \cmidrule(lr){2-4}
        
    %     & & Commutativity & \\
    %     & \myroman{2} & $\psi_1 \land \psi_2 \leftrightarrow \psi_2 \land \psi_1$
    %         & $\phi((q_1 \land q_2), e) = \phi((q_2 \land q_1), e)  $ \\
    %     \cmidrule(lr){2-4}
        
    %     & &  Associativity & \\
    %     & \myroman{3} & $(\psi_1 \land \psi_2) \land \psi_3 \leftrightarrow$
    %         & $\phi((q_1 \land q_2) \land q_3, e) $ \\
    %     & & $\psi_1 \land (\psi_2 \land \psi_3)$
    %         & $= \phi(q_1 \land (q_2 \land q_3), e)$ \\
    % \midrule
    
    % \multirow{9}{*}{$\lor$} 
    %     & & Disjunction  & \\
    %     & & Amplification & \\
    %     & \multirow{2}{*}{\myroman{4}} & $\psi_1 \rightarrow \psi_1 \vee \psi_2$
    %     & $\phi(q_1, e) \leq \phi(q_1 \lor q_2, e) $ \\
    %     % \cmidrule(lr){2-3}
        
    %     & & $\psi_1 \rightarrow \psi_1 \vee \psi_1$
    %     & $\phi(q_2, e) \leq \phi(q_1 \lor q_2, e) $ \\
    %     \cmidrule(lr){2-4}
    
    %     & & Commutativity & \\
    %     & \myroman{5} & $\psi_1 \lor \psi_2 \leftrightarrow \psi_2 \lor \psi_1$
    %         & $\phi((q_1 \lor q_2), e) = \phi((q_2 \lor q_1), e)  $  \\
    %     \cmidrule(lr){2-4}
    %     & & Associativity & \\
    %     & \myroman{6} & $(\psi_1 \lor \psi_2) \lor \psi_3 \leftrightarrow$
    %         & $\phi((q_1 \lor q_2) \lor q_3, e)  $ \\
    %     & & $\psi_1 \lor (\psi_2 \lor \psi_3)$
    %         & $ = \phi(q_1 \lor (q_2 \lor q_3), e)$\\
    % \midrule
    
    % \multirow{4}{*}{$\neg$} 
    %     & & Involution & \\
    %     & \myroman{7} & $\neg \neg \psi_1 \rightarrow \psi_1$ 
    %         & $\phi(q, e) = \phi(\neg \neg q, e)$ \\
    %     \cmidrule(lr){2-4}
        
    %     & & Non-Contradiction & \\
    %     & \myroman{8} & $\psi_1 \land \neg \psi_1 \rightarrow \overline{0}$
    %         & $\phi(q, e) \uparrow \quad \Rightarrow \quad \phi(\neg q, e) \downarrow $\\
    % \bottomrule  
    % \end{tabular}
    % \label{tab:axioms}
    % \end{footnotesize}
    % \end{table}
    

==> tables/properties.tex <==
\begin{table}[h]
\footnotesize
\centering
\caption{Basic properties of conjunction $\land$, disjunction $\lor$, and negation $\neg$ that a logical query embedding model is supposed to possess.
$\conjop, \disjop: [0,1]^d \times [0,1]^d \rightarrow [0,1]^d$ are conjunction and disjunction operator respectively.
$\negop: [0,1]^d \rightarrow [0,1]^d$ is the negation operator.
% $\conjop(\bsq_1, \bsq_2)$, $\disjop(\bsq_1, \bsq_2)$, $\negop (\bsq) \in [0,1]^d$ denote the embedding of $q_1 \land q_2$, $q_1 \lor q_2$, and $\neg q$ respectively.
% $\conjop, \disjop$ denote the conjunction operator and disjunction operator respectively, which take input query embeddings and output embeddings that represent $q_1 \land q_2$ and $q_1 \lor q_2$ respectively.
$\phi(e,q)$ estimates the probability that entity $e$ is an answer to query $q$.}
\begin{tabular}{lll}
\toprule
\multirow{5}{*}{$\land$} 
& Commutativity &
$ \conjop(\bsq_1, \bsq_2)\equiv \conjop(\bsq_2, \bsq_1) $ \\
\cmidrule(lr){2-3}
& Associativitiy &
$\conjop(\conjop(\bsq_1, \bsq_2)), \bsq_3) \equiv \conjop(\bsq_1,  \conjop(\bsq_2,  \bsq_3) $  \\
\cmidrule(lr){2-3}
& Monotonicity &
 $\phi(q_1, e) \geq \phi(q_1, e')$, \\
 & & $\phi(q_2, e) \geq \phi(q_2, e')$\\
& & $\Rightarrow \phi(q_1 \land q_2, e) \geq \phi(q_1 \land q_2, e')$\\
\cmidrule(lr){2-3}
&  & $\phi(q_1 \land q_2, e)) \leq \phi(q_1, e) $\\
&  & $\phi(q_1 \land q_2, e)) \leq \phi(q_2, e) $\\

\midrule
\multirow{3}{*}{$\lor$}
& Commutativity &
$ \disjop(\bsq_1, \bsq_2) \equiv \disjop(\bsq_2, \bsq_1) $ \\
\cmidrule(lr){2-3}
& Associativitiy &
$\disjop(\disjop(\bsq_1, \bsq_2)),\bsq_3) \equiv \disjop(\bsq_1,  \disjop(\bsq_2, \bsq_3)) $  \\
\cmidrule(lr){2-3}
& Monotonicity 
& $\phi(q_1, e) \geq \phi(q_1, e')$, \\
 & & $\phi(q_2, e) \geq \phi(q_2, e')$\\
& & $\Rightarrow \phi(q_1 \lor q_2, e) \geq \phi(q_1 \lor q_2, e')$\\
\cmidrule(lr){2-3}
&  & $\phi(q_1 \lor q_2, e)) \geq \phi(q_1, e) $\\
&  & $\phi(q_1 \lor q_2, e)) \geq \phi(q_2, e) $\\
\midrule
\multirow{2}{*}{$\neg$}
& Involution &
$\negop(\negop (\bsq )) \equiv \bsq$ \\
\cmidrule(lr){2-3}
& Monotonocity
& $\phi(q, e) \geq \phi(q, e')$\\
& & $\Rightarrow \phi(\neg q, e) \leq \phi(\neg q, e') $\\
\bottomrule
\end{tabular}
\label{tab:properties}
\end{table}

==> tables/properties_old.tex <==
\begin{table}[t]
\footnotesize
\centering
\caption{Basic properties of conjunction $\land$, disjunction $\lor$, and negation $\neg$ that a logical query embedding model is supposed to possess.
$\bsq_1 \conjop \bsq_2$, $\bsq_1 \disjop \bsq_2$, $\negop \bsq \in [0,1]^d$ denote the embedding of $q_1 \land q_2$, $q_1 \lor q_2$, and $\neg q$ respectively.
% $\conjop, \disjop$ denote the conjunction operator and disjunction operator respectively, which take input query embeddings and output embeddings that represent $q_1 \land q_2$ and $q_1 \lor q_2$ respectively.
$\phi:[0,1]^d \times [0,1]^d \rightarrow [0,1]$ is a scoring function that predicts the probability that entity $v$ is an answer to query $q$.}
\begin{tabular}{lll}
\toprule
\multirow{5}{*}{$\land$} 
& Commutativity &
$ \bsq_1 \conjop \bsq_2 \equiv \bsq_2 \conjop \bsq_1 $ \\
\cmidrule(lr){2-3}
& Associativitiy &
$(\bsq_1 \conjop \bsq_2) \conjop  \bsq_3 \equiv \bsq_1 \conjop (\bsq_2 \conjop \bsq_3) $  \\
\cmidrule(lr){2-3}
& Monotonicity &
% & & $t( \phi(\be, \bsq_1), \phi(\be, \bsq_2)) \leq t( \phi(\be', \bsq_1), \phi(\be', \bsq_2)) $\\
 $\phi(\be, \bsq_1) \geq \phi(\be', \bsq_1)$, \\
 & & $\phi(\be, \bsq_2) \geq \phi(\be', \bsq_2)$\\
& & $\Rightarrow \phi(\be, \bsq_1 \land \bsq_2) \geq \phi(\be', \bsq_1 \land \bsq_2)$\\
\cmidrule(lr){2-3}
&  & $\phi(\be, \conjop(\bsq_1, \bsq_2)) \leq \phi(\be, \bsq_1) $\\
&  & $\phi(\be, \conjop(\bsq_1, \bsq_2)) \leq \phi(\be, \bsq_2) $\\
% & &$\phi(v, q_1 \land q_2) \geq \phi(v', q_1 \land q_2) $ if $\phi(v, q_1) \geq \phi(v', q_1)$ and $\phi(v, q_2) \geq \phi(v', q_2)$\\

\midrule
\multirow{3}{*}{$\lor$}
& Commutativity &
$ \bsq_1 \disjop \bsq_2 \equiv \bsq_2 \disjop \bsq_1 $ \\
\cmidrule(lr){2-3}
& Associativitiy &
$(\bsq_1 \disjop \bsq_2) \disjop  \bsq_3 \equiv \bsq_1 \disjop (\bsq_2 \disjop \bsq_3) $  \\
\cmidrule(lr){2-3}
& Monotonicity 
& if $\phi(\be, \bsq_1) \geq \phi(\be', \bsq_1)$, \\
& & \quad $\phi(\be, \bsq_2) \geq \phi(\be', \bsq_2)$\\
& &
$\Rightarrow \phi(\be, \bsq_1 \lor \bsq_2) \geq \phi(\be', \bsq_1 \lor \bsq_2)$\\
\cmidrule(lr){2-3}
&  & $\phi(\be, \disjop(\bsq_1, \bsq_2)) \leq \phi(\be, \bsq_1) $\\
&  & $\phi(\be, \disjop(\bsq_1, \bsq_2))\leq \phi(\be, \bsq_2) $\\
\midrule
\multirow{2}{*}{$\neg$}
& Involution &
$\negop(\negop \bsq ) \equiv \bsq$ \\
\cmidrule(lr){2-3}
& Monotonocity
& $\phi(\be, \bsq) \geq \phi(\be', \bsq)$\\
& & $\Rightarrow \phi(\be, \neg \bsq) \leq \phi(\be', \neg \bsq) $\\
\bottomrule
\end{tabular}
\label{tab:properties}
\end{table}

==> tables/querystats.tex <==
\begin{table}[h]
\centering
\caption{Average number of answers of test queries in our new dataset.}
\label{table:querystats}
\begin{tabular}{ccccccccccccccc}
\toprule
   Dataset &  1p &   2p &   3p &  2i &  3i &   ip &   pi &   2u &   up &  2in &  3in &  inp &  pin &  pni \\
\midrule
    %  FB15k & 1.7 & 19.6 & 24.4 & 8.0 & 5.2 & 18.3 & 12.5 & 18.9 & 23.8 & 15.9 & 14.6 & 19.8 & 21.6 & 16.9 \\
 FB15k-237 & 1.7 & 17.3 & 24.3 & 6.9 & 4.5 & 17.7 & 10.4 & 19.6 & 24.3 & 16.3 & 13.4 & 19.5 & 21.7 & 18.2 \\
   NELL995 & 1.6 & 14.9 & 17.5 & 5.7 & 6.0 & 17.4 & 11.9 & 14.9 & 19.0 & 12.9 & 11.1 & 12.9 & 16.0 & 13.0 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/results-EPFO.tex <==
\begin{table*}[t]
\centering
\caption{MRR results (\%) on answering EPFO ($\exists, \land, \lor$) queries.}
\begin{tabular}{ccccccccccc}
\toprule
           Model &  avg &   1p &   2p &   3p &   2i &   3i &   pi &   ip &   2u &   up \\
\midrule
\multicolumn{11}{c}{FB15k} \\ \midrule 
             GQE & 28.0 & 54.6 & 15.3 & 10.8 & 39.7 & 51.4 & 27.6 & 19.1 & 22.1 & 11.6 \\
             Q2B & 38.0 & 68.0 & 21.0 & 14.2 & 55.1 & 66.5 & 39.4 & 26.1 & 35.1 & 16.7 \\
           BetaE & 41.6 & 65.1 & 25.7 & 24.7 & 55.8 & 66.5 & 43.9 & 28.1 & 25.0 & 25.2 \\
 \rowcolor[gray]{.9}   $\modelname_{01}$ &      &      &      &      &      &      &      &      &      &      \\
   \rowcolor[gray]{.9}   \modelname & 43.6 & 64.3 & 32.3 & 27.1 & 55.1 & 66.9 & 46.6 & 38.4 & 34.0 & 27.4  \\
\midrule \multicolumn{11}{c}{FB15k-237} \\ \midrule 
             GQE & 16.3 & 35.0 &  7.2 &  5.3 & 23.3 & 34.6 & 16.5 & 10.7 &  8.2 &  5.7 \\
             Q2B & 20.1 & 40.6 &  9.4 &  6.8 & 29.5 & 42.3 & 21.2 & 12.6 & 11.3 &  7.6 \\
           BetaE & 20.9 & 39.0 & 10.9 & 10.0 & 28.8 & 42.5 & 22.4 & 12.6 & 12.4 &  9.7 \\
\rowcolor[gray]{.9}   $\modelname_{01}$ & 21.7 & 39.8 & 11.5 &  9.1 & 29.6 & 41.7 & 23.6 & 16.1 & 14.2 &  9.7 \\
\rowcolor[gray]{.9}        \modelname & 23.9 & 42.7 & 13.0 & 10.2 & 33.3 & 46.4 & 26.6 & 17.9 & 14.6 & 10.3 \\
\midrule \multicolumn{11}{c}{NELL995} \\ \midrule 
             GQE & 18.6 & 32.8 & 11.9 &  9.6 & 27.5 & 35.2 & 18.4 & 14.4 &  8.5 &  8.8 \\
             Q2B & 22.9 & 42.2 & 14.0 & 11.2 & 33.3 & 44.5 & 22.4 & 16.8 & 11.3 & 10.3 \\
           BetaE & 24.6 & 53.0 & 13.0 & 11.4 & 37.6 & 47.5 & 24.1 & 14.3 & 12.2 &  8.5 \\
 \rowcolor[gray]{.9}  $\modelname_{01}$ & 23.5 & 47.2 & 11.9 & 10.5 & 36.3 & 47.0 & 22.1 & 15.7 & 11.9 &  9.4 \\
  \rowcolor[gray]{.9}      \modelname & 26.8 & 47.3 & 17.2 & 14.3 & 39.1 & 49.8 & 25.9 & 19.9 & 15.4 & 12.3 \\
\bottomrule
\end{tabular}
\label{table:EPFO}
\end{table*}


==> tables/results-logic.tex <==
\begin{table*}[t]
\centering
\caption{MRR results (\%) for three diffrent fuzzy logic systems.}
\begin{tabular}{ccccccc}
\toprule
     Logic & avg (all) &   1p & avg (p) & avg (i) & avg (u) & avg (n) \\
\midrule
\multicolumn{7}{c}{FB15k} \\ \midrule 
     \luka &      30.8 & 68.5 &    41.0 &    47.7 &    23.7 &    13.9 \\
   product &      30.8 & 66.7 &    39.8 &    48.3 &    25.2 &    13.7 \\
    \godel &      31.8 & 65.3 &    41.2 &    49.1 &    26.2 &    14.4 \\
\midrule \multicolumn{7}{c}{FB15k-237} \\ \midrule 
     \luka &      16.9 & 42.4 &    21.7 &    29.9 &    11.4 &     5.9 \\
   product &      17.1 & 42.7 &    21.9 &    30.2 &    12.0 &     5.9 \\
    \godel &      18.1 & 42.7 &    22.0 &    31.0 &    12.5 &     7.6 \\
\midrule \multicolumn{7}{c}{NELL995} \\ \midrule 
     \luka &      20.2 & 51.6 &    28.0 &    33.7 &    12.9 &     7.7 \\
   product &      20.4 & 49.7 &    28.1 &    34.7 &    13.2 &     7.3 \\
    \godel &      20.0 & 47.3 &    26.3 &    33.7 &    13.8 &     7.6 \\
\bottomrule
\end{tabular}
\label{table:logic}
\end{table*}


==> tables/results-negation.tex <==
\begin{table*}[t]
\centering
\caption{MRR and HITS@10 results (\%) on answering FOL queries containing negation. To the best of knowledge, BetaE is the only existing approach that can handle negation in FOL query embedding. }
\begin{tabular}{ccccccccccccc}
\toprule

\multirow{2}{*}{Model} & \multicolumn{6}{c}{MRR} & \multicolumn{6}{c}{HITS@10} \\
\cmidrule(lr){2-7} \cmidrule(lr){8-13}
 &  avg &  2in &  3in &  inp &  pin &  pni &  avg &  2in &  3in &  inp &  pin &  pni \\
      
\midrule  \multicolumn{13}{c}{FB15k} \\ \midrule
      BetaE & 11.8 & 14.3 & 14.7 & 11.5 &  6.5 & 12.4 & 25.3 & 30.8 & 31.9 & 23.4 & 14.3 & 26.3 \\
 \rowcolor[gray]{.9} $\modelname_{01}$ &      &      &      &      &      &      &            &      &      &      &      &      \\
 \rowcolor[gray]{.9} \modelname & 15.9 & 18.3 & 19.8 & 13.9 & 12.1 & 15.4 &            & 32.8 & 33.1 & 25.3 & 20.3 & 28.1 \\
 
 
 \midrule \multicolumn{13}{c}{FB15k-237}   \\ \midrule
      BetaE &  5.4 &  5.1 &  7.9 &  7.4 &  3.5 &  3.4 & 11.9 & 11.3 & 17.3 & 16.0 &  8.1 &  7.0 \\
 \rowcolor[gray]{.9} $\modelname_{01}$ &  6.7 &  7.5 &  9.8 &  6.7 &  4.9 &  5.5 &     12.2       & 12.6 & 16.6 & 14.2 &  8.5 &  9.3 \\
\rowcolor[gray]{.9}  \modelname &  7.6 &  8.5 & 11.6 &  7.8 &  5.2 &  5.8 & 16.0 & 17.0 & 24.2 & 16.6 & 10.7 & 11.4 \\
 
 
 \midrule \multicolumn{13}{c}{NELL995}   \\ \midrule
      BetaE &  5.9 &  5.1 &  7.8 & 10.0 &  3.1 &  3.5 & 12.9 & 11.6 & 18.2 & 20.8 &  6.9 &  7.2 \\
\rowcolor[gray]{.9}  $\modelname_{01}$ &  6.9 &  6.9 &  9.0 &  9.8 &  4.4 &  4.3 &            & 14.6 & 18.8 & 20.3 &  9.1 &  9.0 \\
 \rowcolor[gray]{.9} \modelname &  7.6 &  7.7 &  9.5 & 10.9 &  4.8 &  5.3 & 15.6 & 16.8 & 22.8 & 16.1 & 10.6 & 11.6 \\
\bottomrule
\end{tabular}
\label{table:negation}
\end{table*}


==> tables/semantics.tex <==
\begin{table}[h]
\footnotesize
\centering
\caption{
Semantics of classical logic and fuzzy logic.
$I(\varphi)$ $\phi(q,e), q[e] \equiv \varphi$
}
\begin{tabular}{lll}
\toprule
 &  Classical Logic & \godel~Logic \\
\midrule
Interpretation $I$
    & $I: F_{mL} \rightarrow \{0,1\}$
    & $I: F_{mL} \rightarrow [0,1]$
    \\
\midrule
$I(\varphi \land \psi)$
    & $\min(I(\varphi), I(\psi))$
    & $\min(I(\varphi), I(\psi))$
    \\
\midrule
$I(\varphi \lor \psi)$
    & $\max(I(\varphi), I(\psi))$
    & $\max(I(\varphi), I(\psi))$
    \\
\midrule
$I(\varphi \rightarrow \psi)$
    & 
        $\left\{
             \begin{array}{lr}
             1, \quad \text{if}~I(\varphi) \leq I(\psi)  \\
             I(\psi), \quad \text{otherwise}
             \end{array}
        \right.
        $
    & 
        $\left\{
             \begin{array}{lr}
             1, \quad \text{if} I(\varphi) \leq I(\psi)  \\
             I(\psi), \quad \text{otherwise}
             \end{array}
        \right.
        $
    \\
    
\midrule
$I(KB \rightarrow \psi)=1,$
$I(KB \rightarrow \psi')<1$
    & 
        $\left\{
             \begin{array}{lr}
             1, \quad \text{if}~I(\varphi) \leq I(\psi)  \\
             I(\psi), \quad \text{otherwise}
             \end{array}
        \right.
        $
    & 
        $\left\{
             \begin{array}{lr}
             1, \quad \text{if} I(KB) \leq I(\varphi)  \\
             I(\psi), \quad \text{otherwise}
             \end{array}
        \right.
        $
    \\
    
\midrule
$I(KB \rightarrow \psi) \geq I(KB \rightarrow \psi')$
    & 
        $
        I(\psi) \geq I(\psi')
        $
    & 
            $
        I(\psi) \geq I(\psi')
        $

    \\
    
    
\midrule
$I(\neg \varphi)$
    & $I(\psi \rightarrow \overline{0})$
    & $I(\psi \rightarrow \overline{0})$
    \\
    


\bottomrule  
\end{tabular}
\label{tab:semantics}
\end{table}

==> writeup/7-B-ablationstudy.tex <==

\newpage
\clearpage
\section{Case Study} \label{ap:FOL-def}

Table \ref{tab:casestudy} gives an example of query answering on FB15k-237 using \modelname.

\begin{table}[h]
    % \scriptsize
    \footnotesize
    \centering
    \caption{
    Examples of $2p$ query answering on FB15k-237 using \modelname. 
    We show 3 entities that rank top among all the entities. We also show the top 3 entities under the \emph{filtered} setting, where answers that can be found by scanning training edges are filtered out from ranking.
    % Answers that can be found by scanning training edges are filtered out from ranking.
    \emph{Easy} indicates whether the answer can be found by scanning the training edges.
    % Due to KG incompleteness, some answers may be in fact correct but cannot be discovered by traversing the KG.
    }
    \begin{tabular}{clllll}
    \toprule
    Type & Query &  Predicted Answer & Correct & Easy\\
    \midrule
    \multirow{3}{*}{2p}
        & Which country have won Olympics Godel Medals? 
        
        & United States of America
        & Yes
        & Yes
        \\

    & q=$V_?$: $\exists V_1$: wonByAthlete(Olympics Godel Medal, $V_1$) 
        & Europe
        & No
        & No
        \\

    & $\land$ personAffiliatedWithCountry($V_1$, $V_?$)
        & United Kingdom
        & Yes
        & Yes
        \\

    & 
        & China
        & Yes
        & Yes
        \\

    & 
        & Canada
        & Yes
        & No
        \\
    \midrule
    \multirow{3}{*}{2i}
        & Which film has both Jude Law and Natalie Portman?
        
        & Closer
        & Yes
        & No
        \\

    & q=$V_?$: personInFilm(Jude Law, $V_?$) 
        & Sherlock Holmes
        & No
        & No
        \\

    & $\land$ personInFilm(Natalie Portman, $V_?$) 
        & Sherlock Holmes 2
        & No
        & No
        \\

    & 
        & Black Swan
        & No
        & No
        \\

    & 
        & The Holiday
        & No
        & No
        \\

    \bottomrule  
    \end{tabular}
    \label{tab:casestudy}
    \end{table}



==> writeup/outline.tex <==

%outline
\begin{markdown}
- Multi-hop KG reasoning
    - QGE, Query2Box, EmQL
        - They can only model EPFO queries. Cannot handle negation.
    - BetaE 
    
- T-norm based logic and fuzzy set
    - Lukasiewicz, Godel, product logic
    - Examples of applications: probabilistic soft logic

\end{markdown}


% outline
\begin{markdown}
- Background
    - Knowledge graphs (KGs), Reasoning on KGs, FOL queries
    - Examples of FOL queries
    
- Challenges
    - Incompleteness of KGs
        - Sub-graph matching cannot deal with missing facts. Need embedding models
    - Preserve the properties of logical operators in the embedding space
    
- Literature review
    - Main idea
        - Computation graph: leaf nodes for anchor entities, root node for query
        - Every internal node is considered as a set. Logical operators are implemented using corresponding set operations
        - Generate query embedding, match with entity embedding
    - Methods
        - GQE, Query2Box, EmQL 
            - Can only handle Existential Positive First-Order (EPFO) queries. Unable to handle negation
        - BetaE (Able to model negation)
            - Negation: not strict. Does not satisfy fuzzy set complement axioms (monotonicity). Far from perfect performance.
            - Union (Disjunction):
                - DNF: Exponential complexity in the worst case
                - DM: Restricted by the modality of Beta distributions. Either unimodal or bimodal.
- Our method
    - Entity represented as probabilities and relation as transforms
        - Motivation: Entities consist of various properties (e.g. color), and we therefore represent them by its Bernoulli probabilities on latent properties.
    - Queries considered as fuzzy sets. Define logical operators based on t-norms
        - Motivation: Preserve the logical operator properties in the embedding space
    - Our set operations satisfy the axioms of fuzzy set axioms
    - End-to-end differentiable model that could train for any operators
\end{markdown}





% % outline
\begin{markdown}
- ;Knowledge graphs
    - ;notations
- ;Definition for FOL queries
- ;Computation graph
- Fuzzy set and t-norms
    - fuzzy set theory (conjunction as t-norm, disjunction as t-conorm)
    - basic properties of t-norms
    - 3 basic t-norms
    - t-norms and the corresponding t-conorms
\end{markdown}



\begin{markdown}

- Entity representation

- Query representation

% - Entity representation (two possible choices)
%     - Discrete representation
%     - Continuous representation
%     - Discussion about how it affects the theory proving
    
- Scoring function for $P(e|S)$
\end{markdown}

    


==> writeup/trash.tex <==
Particularly, we present \modelname~with reference to product logic, one of the most prominent fuzzy logic systems \cite{KlementTNormBook}.
Alternative design choices based on \luka~and \godel~logic are discussed in Appendix \ref{ap:tnorm}.
The embeddings of $q_1 \land q_2$, $q_1 \lor q_2$, and $\neg q$ are computed as follows:
\begin{alignat*}{2}
        q_1 \land q_2: & \quad \conjop(\bsq_1, \bsq_2) && =   \bsq_1 \circ \bsq_2 \\
        q_1 \lor q_2: & \quad \disjop(\bsq_1, \bsq_2) && = \bsq_1 + \bsq_2 - \bsq_1 \circ \bsq_2 \\
        \neg q: & \quad \negop(\bsq) && = \mathbf{1} - \bsq
\end{alignat*}
where 
$\circ$ denotes element-wise multiplication (fuzzy conjunction), $\mathbf{1}$ is the all-ones vector, and $\conjop, \disjop, \negop$ denote the embedding based logical operators respectively. 

% \shirley{Omit the other two logic systems due to space limit.}
% \paragraph{Logical Connectives ($\land, \lor, \neg)$}
% We propose to use fuzzy logic operations to model logic connectives in vector space.
% \begin{alignat*}{2}
%     q_1 \land q_2: & \quad \conjop(\bsq_1, \bsq_2) && =   \bsq_1 \circ \bsq_2 \\
%     q_1 \lor q_2: & \quad \disjop(\bsq_1, \bsq_2) && = \bsq_1 + \bsq_2 - \bsq_1 \circ \bsq_2 \\
%     \neg q: & \quad \negop(\bsq) && = \mathbf{1} - \bsq
% \end{alignat*}
% Following product logic with \luka~negator \cite{KlementTNormBook}, 


% \section{Additional Experimental results}
% \subsection{Different logic systems} \label{ap:otherlogic}
% Based on the three \tnorms~listed in Table \ref{tab:tnorms}, we define the three sets of intersection and union operators, namely \godel, product, and \luka~logic as follows:
% \begin{align*}
%   \text{\godel:}  & \mathcal{I}(\Svec_1, \Svec_2)=\bot (\Svec_1, \Svec_2) \\
%     & \mathcal{U}(\Svec_1, \Svec_2)=\top (\Svec_1, \Svec_2) \\
%   \text{Product:}  & \mathcal{I}(\Svec_1, \Svec_2)=\Svec_1 \circ \Svec_2 \\
%     & \mathcal{U}(\Svec_1, \Svec_2)=\Svec_1+\Svec_2 - \Svec_1 \circ \Svec_2\\
%   \text{\luka:}  & \mathcal{I}(\Svec_1, \Svec_2)= \top (\Svec_1+\Svec_2-1, \mathbf{0})\\
%     & \mathcal{U}(\Svec_1, \Svec_2)=\bot (\Svec_1+\Svec_2-1, \mathbf{1})
% \end{align*}
% where $\bot$ and $\top$ denote element-wise minimum and maximum respectively, $\circ$ is the element-wise product, and $\mathbf{0}$ and $\mathbf{1}$ are the all-zeros and all-ones vector respectively.
% Note that our logical operator do not require learning any parameters, which is an outstanding advantage when only KG triples are available for training.

% MRR results are reported in Table \ref{table:logic}.

% Here we list some additional experimental results in Table \ref{table:EPFO}, \ref{table:1p}, and \ref{table:logic}.
% \input{tables/results-logic}
% \input{tables/results-EPFO}
% \input{tables/results-negation}



% \section{Axiomatic system of fuzzy set theory}
% \label{sec:fuzzyaxioms}

% \citet{fuzzysetAxioms} connected fuzzy set theory with fuzzy logic systems and argued that the fuzzy set intersection can be interpreted as "logical and", the union as "logical or", and the fuzzy set $\tilde{S}$ as the statement "The element $x$ belongs to set $\tilde{S}$", which can be accepted as more or less true.
% Considering two statements $S$ and $T$, for which the truth values are $\mu_S$ and $\mu_T$, respectively, $\mu_S, \mu_T \in [0,1]$.
% The truth value of "and" and "or" combination of these statements $\mu_{S \land T}$ and $\mu_{S \lor T}$, both from the interval $[0,1]$, are interpreted as the values of the membership functions of the intersection and union of $S$ and $T$.

% Referring to the logic systems, \citeauthor{fuzzysetAxioms} proposed the following axioms for the intersection operator $f$ and union operator $g$ of fuzzy sets:
% \begin{enumerate}
%     \item $f(1,1)=1$ and $g(0,0)=0$
%     \item Continuity and Monotonicity: $f$ and $g$ are non-decreasing and continuous in $[0,1]$
%     \item Commutativity: $f$ and $g$ are symmetric, that is,
%         \begin{align*}
%             f(\mu_S, \mu_T) &= f(\mu_T, \mu_S)\\
%             g(\mu_S, \mu_T) &= g(\mu_T, \mu_S)
%         \end{align*}
%     \item Associativity: 
%         \begin{align*}
%             f(\mu_S, f(\mu_{T_1}, \mu_{T_2}))=f(f(\mu_S, \mu_{T_1}), \mu_{T_2})\\
%             g(\mu_S, g(\mu_{T_1}, \mu_{T_2})=g(g(\mu_S, \mu_{T_1}), \mu_{T_2}))
%         \end{align*}
%     \item $f(\mu_S, \mu_T) \leq \min(\mu_S, \mu_T)$ and $g(\mu_S, \mu_T) \geq \max(\mu_S, \mu_T)$. This implies that accepting the truth of statement $S \land T$ requires more, and accepting the truth of $S \lor T$ less than accepting S or T alone as true.
% \end{enumerate}

% Additionally, \citeauthor{fuzzysetAxioms} proposed that the complement function $h$ should also be continuous, monotonically decreasing, and involutory, i.e. $h(h(x))=x$.

% In addition to the widely accepted axiomatic system of \citeauthor{fuzzysetAxioms}, others axiomatic systems have been proposed for fuzzy set theory (e.g. by \citet{hamacher1978sensitivity}).
% We refer interested readers to \cite{fuzzytheorybook} for more information.



% \subsection{Fuzzy Set Theory}
% \begin{markdown}
% **Axioms for fuzzy set operations**\\
% **Fuzzy complement (negation)**

% $c: [0,1] \rightarrow [0,1]$

% - Boundary condition $c(0)=1, c(1)=0$
% - Monotonicity $\forall a,b \in [0,1]$, if $a<b$ then $c(a)>c(b)$
% - Continuity
% - Involutions $c(a)=a$

% **Fuzzy intersection (conjunction)**

% $i: [0,1] \times [0,1] \rightarrow [0,1]$

% - Boundary condition $i(a,1)=a$
% - Monotonicity if $b\leq d$ then $i(a,b)\leq i(a,d)$
% - Commutativity $i(a,b)=i(b,a)$
% - Associativity $i(a, i(b,d))=i(i(a,b),d)$
% - Continuity
% - Subidempotency $i(a,a) \leq a$
% - Strict monotonicity 
% \end{markdown}
%      $i(a_1, b_1) \leq i(a_2, b_2)$ if $a_1 \leq a_2, b_1 \leq b_2$
     
% \begin{markdown}
% **Fuzzy union (disjunction)**

% $u: [0,1] \times [0,1] \rightarrow [0,1]$

% - Boundary condition $u(a,0)=u(0,a)=a$
% - Monotonicity if $b\leq d$ then $u(a,b)\leq u(a,d)$
% - Commutativity $u(a,b)=u(b,a)$
% - Associativity $u(a, u(b,d))=u(u(a,b),d)$
% - Continuity
% - Subidempotency $u(a,a) \geq a$
% - Strict monotonicity 
% \end{markdown}
%      $i(a_1, b_1) \leq i(a_2, b_2)$ if $a_1 \leq a_2, b_1 \leq b_2$

% \begin{markdown}
% ### t-norm
% A t-norm is a function $T: [0, 1] \times [0, 1] \rightarrow [0, 1]$ which satisfies the following properties:

% * Boundary condition: $T(a, 1) = a$
% * Commutativity: $T(a, b) = T(b, a)$
% * Monotonicity: $T(a, b) \leq T(c, d)$ if $a \leq c$ and $b \leq d$
% * Associativity: $T(a, T(b, c)) = T(T(a, b), c)$

% ### t-conorm
% A t-conorm is a dual function of a t-norm defined by De Morgan's law and the negator $c(x)=1-x$:
% $s(a,b) = 1 - t(1-a, 1-b)$ 

% A t-conorm satisfies the following properties:

% * Boundary condition: $s(a, 0) = a$
% * Commutativity: $s(a, b) = s(b, a)$
% * Monotonicity: $s(a, b) \leq s(c, d)$ if $a \leq c$ and $b \leq d$
% * Associativity: $s(a, s(b, c)) = s(s(a, b), c)$

% \end{markdown}


% \input{writeup/outline}



% For a valid query, its computation graph is a directed acyclic graph (DAG), with the anchor nodes as the source nodes of the DAG and the query target as the unique sink node (i.e. the tree root).



% \section{Theoretical analysis} \label{ap:analysis}

% \subsection{Fully Expressiveness}

% Let
% \begin{align}
% \phi_e = [0, ..., 0, 1, 0,..., 0], \phi_e(i) = 1\\
% \phi_{e'} = [0, ... 0, 1, 0,..., 0], \phi_{e'}(j) = 1\\
% \end{align}


% Objective:

% \begin{align*}
% & \text{If}\\
% & \phi_{S_1}(i) \geq \phi_{S_1}(j) \\
% & \phi_{S_2}(i) \geq \phi_{S_2}(j)\\
% & \text{Then}\\
% & f_\land(\phi_{S_1}, \phi_{S_2})(i) \geq f_\land(\phi_{S_1}, \phi_{S_2})(j)  \label{conc-point}
% \end{align*}


% ### [1] Godel Logic

% #### Definition

% $$
% f_\land(x,y) = min(x,y) \\
% $$

% #### Proof

% \begin{align}
% f_\land(\phi_{S_1}, \phi_{S_2})(i) = min(\phi_{S_1}(i), \phi_{S_2}(i))\\
% \geq min(\phi_{S_1}(j), \phi_{S_2}(j)) = f_\land(\phi_{S_1}, \phi_{S_2})(j)
% \end{align}

% Eq $\ref{conc-point}$ is satisfied.



% ### [2] Lukasiewicz Logic

% #### Definition

% $$
% f_\land(x,y) = max(x+y-1,0)
% $$

% #### Proof

% \begin{align}
% f_\land(\phi_{S_1}, \phi_{S_2})(i) = max(\phi_{S_1}(i)+\phi_{S_2}(i)-1, 0)\\
% \geq max(\phi_{S_1}(j)+\phi_{S_2}(j)-1, 0) = f_\land(\phi_{S_1}, \phi_{S_2})(j)
% \end{align}

% Eq $\ref{conc-point}$ is satisfied.



% ### [3] Product Logic

% #### Definition

% $$
% f_\land(x,y) = xy
% $$

% #### Proof

% \begin{align}
% f_\land(\phi_{S_1}, \phi_{S_2})(i) = \phi_{S_1}(i) \phi_{S_2}(i) \\
% \geq \phi_{S_1}(j) \phi_{S_2}(j) = f_\land(\phi_{S_1}, \phi_{S_2})(j)
% \end{align}






% \YS{citations} 
and adapts to complex FOL queries by gradient-based optimization or beam search. 
% The constant-time dense search based inference cannot be applied, since CQD does not provide a query embedding in the same space as the entity.
Its inference involves scoring all the entities for each atom query, which is highly undesirable in real-world applications and can lead to query timeout described earlier.
This time estimate \YS{which time estimate?} has not even taken into account the overhead of gradient descent and beam search.
% to While they attempt to constrain intermediate result size by using gradient-based vector representation or beam search, gradient descent optimization and beam search bring additional overhead. 
However, its inference still unfortunately involves scoring all the entities for each atom query, which is highly undesirable in real-world applications.
In addition, accuracy of such link prediction based models is also limited by the performance of KG link prediction, as they cannot take advantage of complex query training samples.


Recent work CQD \cite{CQD} proposes to train an embedding based KG Completion model (e.g. ComplEx \cite{ComplEx}) to impute missing edges.

(e.g. the associative law $ (\varphi \land \psi) \land \chi \equiv \varphi \land (\psi \land \chi)$ for logical formulae $\varphi, \psi, \chi$), 

% They can be divided into two categories: logical query embedding methods and link prediction based techniques.
% recent works leverage embeddings to conduct logical query answering, which can be categorized into logical query embedding methods and link prediction based methods.
% In order to efficiently answer complex logical queries on KG while generalize for missing edges, 
% They seek to embed logical queries and entities in the same vector space and conduct query answering via dense similarity search.

% and merge results using \emph{t-norms} and \emph{t-conorms}.
% predictionmodel and adapts to complex FOL queries in the inference stage by gradient-based optimization or beam search. 
% % The constant-time dense search based inference cannot be applied, since CQD does not provide a query embedding in the same space as the entity.
% Its inference involves scoring all the entities for each atom query, which is highly undesirable in real-world applications and can lead to query timeout described earlier.
% This time estimate has not even take into account the overhead of gradient descent and beam search.
% In addition, accuracy of such link prediction based models is also limited by the performance of KG link prediction, as they cannot take advantage of complex query training samples.

% Classical methods search the KG to retrieve entities for sub-queries and then merge intermediate results \cite{lei2011rdfsubgraph, schmidt2010foundations}.
% through methods such as subgraph matching
% This task poses a number of challenges. 
% A straightforward solution is to search the KG and merge intermediate results through methods such as subgraph matching \cite{lei2011rdfsubgraph, schmidt2010foundations}.
% However, such approaches have drawbacks in terms of computation complexity and robustness to missing edges of KGs.
% The computational complexity for walking on KG grows exponentially with the complexity of the query and is drastically affected by the size of the intermediate results, making such methods hard to scale to modern KGs. 
% One possible solution consists in computing all missing entries via KG completion methods \cite{TransE, DistMult, ComplEx, RotatE}, but this would further exacerbate the former issue.

Given a relation $r$ and the anchor entity embedding $\be$, we model the query embedding 
as the following relation transform:


The key idea is to implement logical operation in a differentiable way and embed a complex logical query by iteratively computing embedding from leaf nodes to root node according to the computation graph (Figure \ref{fig:computation_graph}). 
\modelname achieves by 3.3\% absolute (ca. 15.8\% relative) performance improvement of MRR score on FB15k-237 and 4.7\% absolute (ca. 19.1\% relative) improvement on NELL995. 

\subsection{Model Learning and Inference}
comparing to the best baseline BetaE \cite{BetaE} 
\modelname achieves by 3.3\% absolute (ca. 15.8\% relative) performance improvement of MRR score on FB15k-237 and 4.7\% absolute (ca. 19.1\% relative) improvement on NELL995. 

Given a query embedding $q$, 
we seek to maximize the following expectations:
\begin{align}
    & \mathbb{E}[e \in \llbracket q \rrbracket] \label{eq:losspos1} \\
    & \mathbb{E}[e \in \llbracket q \rrbracket \cap \{e\}] \label{eq:losspos2} \\
    & \mathbb{E}[e \in \llbracket q \rrbracket] \cup \{e\}] \label{eq:losspos3}
\end{align}
and minimize the following expectations:
\begin{align}
    & \mathbb{E}[e' \in \llbracket q \rrbracket] \label{eq:lossneg1} \\
    & \mathbb{E}[e \in (\llbracket q \rrbracket)^{\complement}] \label{eq:lossneg2}
\end{align}
[formulation of $\{e\}$]
where $e$ is an answer entity to $q$, $e' \notin \llbracket q \rrbracket$ represents a random negative sample, and
$\cap, \cup, (\cdot)^{\complement}$ denote set intersection, union, and complement respectively.
Including Eq. (\ref{eq:losspos2})(\ref{eq:losspos3})(\ref{eq:lossneg2}) is the self-supervised learning strategy that provides additional supervision for logical operators. 
Accordingly, the objective function is defined as follows:
\begin{equation*}
    L= - \sum_{s_{+}} \lambda_{s+} \log \sigma(s_{+} - \gamma)
    - \sum_{s_{-}} \lambda_{s-}  \log \sigma(\gamma - s_{-})
\end{equation*}
where $s_{+}$ denotes the score we want to maximize, i.e. Eq. (\ref{eq:losspos1},\ref{eq:losspos2},\ref{eq:losspos3}); and $s_{+}$ denotes the score we want to minimize, i.e. Eq. (\ref{eq:lossneg1},\ref{eq:lossneg2}). $\lambda$ represents a loss term weight, with $\sum_{s_{+}} \lambda_{s+}=1$ and $\sum_{s_{-}} \lambda_{s-}=1$.


While they attempt to constrain intermediate result size by using gradient-based vector representation or beam search, gradient descent optimization and beam search bring additional overhead. Furthermore, its inference unfortunately involves scoring all the entities for each atom query, which is highly undesirable in real-world applications and can lead to query timeout described earlier.

% The motivation is that the union of multiple boxes is no longer a box, so they want to do this only at the last step.
% This approach has the advantage of allowing the disjunction operation to be performed as long as the model defines a conjunction operation. 
% The advantage of this approach is that the disjunction operation can be performed as long as the model defines a conjunction operator. 

They can be divided into two categories: logical query embedding methods and link prediction based techniques.
% recent works leverage embeddings to conduct logical query answering, which can be categorized into logical query embedding methods and link prediction based methods.
% In order to efficiently answer complex logical queries on KG while generalize for missing edges, 
Logical query embedding methods \cite{GQE, Query2Box, BetaE} seek to embed logical queries and entities in the same vector space and conduct query answering via dense similarity search.


While an alternative way is to train a link prediction model with only KG edges and impute missing edges in the inference stage, these models face severe scalability difficulties. 
For example, CQD \cite{CQD} trains a ComplEx \cite{ComplEx} link predictionmodel and adapts to complex FOL queries in the inference stage by gradient-based optimization or beam search. 
% The constant-time dense search based inference cannot be applied, since CQD does not provide a query embedding in the same space as the entity.
Its inference involves scoring all the entities for each atom query, which is highly undesirable in real-world applications and can lead to query timeout described earlier.
This time estimate has not even take into account the overhead of gradient descent and beam search.
In addition, accuracy of such link prediction based models is also limited by the performance of KG link prediction, as they cannot take advantage of complex query training samples.

This task poses a number of challenges. 
A straightforward solution is to search the KG and merge intermediate results through methods such as subgraph matching \cite{lei2011rdfsubgraph, schmidt2010foundations}.
However, such approaches have drawbacks in terms of computation complexity and robustness to missing edges of KGs.
The computational complexity for walking on KG grows exponentially with the complexity of the query and is drastically affected by the size of the intermediate results, making such methods hard to scale to modern KGs. 
% For example, 
Wikidata, one of the most influential KGs, reports that their query engine performance falls off a cliff and may time out, when the number in a group of interest (for example, people born in France) exceeds a certain threshold 
% \cite{wikidataqueryplan} 
\footnote{\url{https://www.wikidata.org/wiki/Wikidata:SPARQL_query_service/query_optimization}}.
Furthermore, KGs in the real-world are often severely incomplete, and this makes it impossible to answer many queries directly by searching KGs.
% One possible solution consists in computing all missing entries via KG completion methods \cite{TransE, DistMult, ComplEx, RotatE}, but this would further exacerbate the former issue.

This task poses a number of challenges. 
A straightforward solution is to search the KG and merge intermediate results through methods such as subgraph matching \cite{lei2011rdfsubgraph, schmidt2010foundations}.
However, such approaches have drawbacks in terms of computation complexity and robustness to missing edges of KGs.
The computational complexity for walking on KG grows exponentially with the complexity of the query and is drastically affected by the size of the intermediate results, making such methods hard to scale to modern KGs. 
% For example, 
Wikidata, one of the most influential KGs, reports that their query engine performance falls off a cliff and may time out, when the number in a group of interest (for example, people born in France) exceeds a certain threshold 
% \cite{wikidataqueryplan} 
\footnote{\url{https://www.wikidata.org/wiki/Wikidata:SPARQL_query_service/query_optimization}}.
Furthermore, KGs in the real-world are often severely incomplete, and this makes it impossible to answer many queries directly by searching KGs.

% Traditional symbolic reasoning \cite{lei2011rdfsubgraph, schmidt2010foundations} have drawbacks in terms of computation complexity and handling missing edges of KGs.
As a remedy to these issues, recent works utilize embedding models to answer logical queries. They can be divided into two categories: logical query embedding methods and link prediction based techniques.
% recent works leverage embeddings to conduct logical query answering, which can be categorized into logical query embedding methods and link prediction based methods.
% In order to efficiently answer complex logical queries on KG while generalize for missing edges, 
Logical query embedding methods \cite{GQE, Query2Box, BetaE} seek to embed logical queries and entities in the same vector space and conduct query answering via dense similarity search.
The key idea is to implement logical operation in a differentiable way and iteratively compute embedding from leaf nodes to root node according to the computation graph (Figure \ref{fig:computation_graph}).
Such approaches are promising in handling missing edges and offers significant advantages in terms of time and space complexity of inference, since they do not need to track intermediate entities. These models reduce this problem to dense similarity search (e.g. nearest neighbor search), and therefore its inference could be performed efficiently by methods like locality sensitive hashing \cite{indyk1998approximate}.
However, the logic operators in these models are defined in an ad-hoc fashion, many of which do not satisfy the basic logic laws (e.g. $ (\varphi \land \psi) \land \chi \equiv \varphi \land (\psi \land \chi)$),
% axiomatic system of classical logic or fuzzy logic \cite{KlementTNormBook}, 
which limits their inference accuracy. 
Furthermore, the logical operators of existing works are based on deep architectures, which requires a large number of training queries containing such logic operations to learn the parameters. This greatly limits the scope of application of the models,
since it is challenging to collect a large number of reasonable complex queries with accurate answers.
While an alternative way is to train a link prediction model with only KG edges and impute missing edges in the inference stage, these models face severe scalability difficulties. 
For example, CQD \cite{CQD} trains a ComplEx \cite{ComplEx} link predictionmodel and adapts to complex FOL queries in the inference stage by gradient-based optimization or beam search. 
% The constant-time dense search based inference cannot be applied, since CQD does not provide a query embedding in the same space as the entity.
Its inference involves scoring all the entities for each atom query, which is highly undesirable in real-world applications and can lead to query timeout described earlier, since the number of entities in real-world KGs are often in millions \cite{bollacker2008freebase, Wikidata2014}.
This time estimate has not even take into account the overhead of gradient descent and beam search.
In addition, accuracy of such link prediction based models is also limited by the performance of KG link prediction, as they cannot take advantage of complex query training samples.

Our objective is to create a model that addresses the above issues. A good FOL query answering model should be able to embed arbitrary FOL logical queries, handle missing edges robustly, and perform constant time inference. 
The logic operators must be consistent with the axioms of classical logic. In addition, the model should be able to generalize to complex query models when only KG edges are available for training.

We hereby present \modelname~(\underline{Fuzz}y \underline{Q}uery \underline{E}mbedding), a fuzzy logic based embedding framework for answering logical queries on KGs.
We borrow the idea of fuzzy logic and use the fuzzy conjunction, disjunction, and negation operations 
% to define the logical operators in vector space 
to implement logical operators in a more principled and learning-free manner.
Moreover, We introduce self-supervised learning into the training process in light of logical laws like $\varphi \land \varphi \equiv \varphi$ ($\varphi$ is a logical formula). This allows our model to be trained with logical operators even in the absence of a complex FOL query training set and thus further improves its ability to generalize effectively to new query structures.

We first discuss how to embed an atomic query like $\emph{Compose}(\emph{John Lennon}, V_?)$.
% , which is essentially representing the target variable $V_?$.
% Specifically, the objective is to derive a query embedding for the variable $V_?$  given the anchor entity embedding $\be_{\text{John Lennon}}$ and the relation representation of \emph{Compose}.
In our work, we associate each relation $r \in \mathcal{R}$ with a weight matrix $\mathbf{W}_r \in \mathbb{R}^{d \times d}$ and a bias vector $\mathbf{b}_r \in \mathbb{R}^d$.
% //TODO: update e to variable
Given a relation $r$ and the anchor entity embedding $\be$, we model the query embedding 
as the following relation transform:


% During training, we optimize the ranking-based objective for each dimension in order to ensure that \modelname~fulfills the properties in Table \ref{tab:axioms}.
% We optimize the ranking-based objective for each dimension during training, ensuring that for each dimension, \modelname~satisfy the above properties of logical operations.
To implement the embedding of entities and queries to the fuzzy space of $[0,1]^d$, we consider two mapping functions
\input{writeup/3-preliminaries}

\paragraph{Scoring Function}
% Given a query $q$ and an entity $e$, $\phi(q,e)$ evaluates the truth value of the FOL formula when replacing the target variable in $q$ with $e$.
% With $\be, \bsq \in [0,1]^d$, 
We estimate the plausibility that $e$ answers $q$ by dot product:
% $\phi(q, e) =  \be^\intercal \bsq$.
\begin{equation} \label{eq:scoring}
  \phi(q, e) =  \bsq^\intercal \be
    % \phi(q, e) = \text{LN}(\bsq)^\intercal \text{LN}(\be)
\end{equation}
% where $LN$ is Layer Normalization \cite{LayerNorm}.
% $\phi(q, e) = \sigma( \bsq^\intercal \be )$.
In practice, multiple conjunction operations tend to diminish the norms of query embeddings. In order to mitigate the influence of query complexity, we apply Layer Normalization \cite{LayerNorm} before computing the score.


Our objective is to design a query embedding model that can fit the axiomatic system of classical logic and retain the properties in Table \ref{tab:axioms}. 
Considering fuzzy logic systems is a natural direction, as their axiomatic systems are fully compatible with classical logic, and their logical operations therefore conform to these properties as well. 
Furthermore, fuzzy logic allows values to float between $[0,1]$, which allows us to design end-to-end differentiable logic operators as opposed to $0,1$ Boolean logic.
% A natural direction is to consider fuzzy logic systems, as their axiomatic systems are fully compatible with classical logic, and their logical operations therefore conform to these properties as well. 
In our work, we implement the logical operators in vector space through element-wise fuzzy conjunction, fuzzy disjunction and fuzzy negation.
This design ensures that we can satisfy the requirements of Table \ref{tab:axioms} in all dimensions.
Particularly, we present \modelname~with reference to product logic, one of the most prominent fuzzy logic systems \cite{KlementTNormBook}.
Alternative design choices based on \luka~and \godel~logic are discussed in Appendix \ref{ap:tnorm}.


\paragraph{Embedding Space} 
We propose to embed entities and queries into the same space: $\be, \bsq \in [0,1]^d$.
Using this embedding space provides the following benefits:
(i) Each dimension of the embedding vector is between $[0,1]$, which satisfies the domain and range requirements of fuzzy logic and allows the model to execute element-wise fuzzy conjunction/disjunction/negation.
(ii) The representation is endowed with probabilistic interpretation.
Particularly, this domain restriction is implemented with an element-wise sigmoid function.

\paragraph{Atomic Query}
We first discuss how to embed an atomic query like $\emph{Compose}(\emph{John Lennon}, V_?)$.
% , which is essentially representing the target variable $V_?$.
% Specifically, the objective is to derive a query embedding for the variable $V_?$  given the anchor entity embedding $\be_{\text{John Lennon}}$ and the relation representation of \emph{Compose}.
In our work, we associate each relation $r \in \mathcal{R}$ with a weight matrix $\mathbf{W}_r \in \mathbb{R}^{d \times d}$ and a bias vector $\mathbf{b}_r \in \mathbb{R}^d$.
Given a relation $r$ and the anchor entity embedding $\be$, we model the query embedding 
% for the target variable $V_?$ 
as the following relation transform:
\begin{equation*}
\footnotesize
    \bsq = \mathcal{P}_r(\be) = \boldsymbol{\sigma}( \text{LN}( \mathbf{W}_r \be + \mathbf{b}_r))
\end{equation*}
where $\boldsymbol{\sigma}$ is an element-wise sigmoid function to impose the domain restriction $\bsq \in [0,1]^d$.
To avoid the rapid growth in number of parameters with the number of relations and alleviate overfitting on rare relations, we follow \cite{RGCN} and adopt \emph{basis-decomposition} to define $W_r$: 
\begin{equation*}
    \mathbf{W}_r = \sum_{i=1}^{m} a_{ri}\mathbf{M}_i
\end{equation*}
i.e. as a linear combination of $m$ basis transformations $\mathbf{M}_i \in \mathbb{R}^{d \times d}$ with coefficients $a_{ri}$ that depend on $r$. It can be seen as a form of effective weight sharing among different relation types. Note that intermediate variables can be embeded by performing multiple
such transformations.

% and \modelname~can therefore handle existential quantifier.
% Take the following query that \emph{finds all the artists who have sung songs composed by John Lennon} as an example:
% \begin{equation*}
%     q[V_?] = \exists V~\emph{Compose(John Lennon}, V) \land \emph{SungBy}(V, V_?)
% \end{equation*}
% It is embeded as
% $\bsq = \mathcal{P}_{\text{SungBy}}(\mathcal{P}_{\text{Compose}}(\be_{\text{John Lennon}}))$.

\paragraph{Existential Quantifier ($\exists$)}
An FOL query may involve bound variables introduced by Existential Quantifier ($\exists$).
A query involving existential quantified variables can be embeded by performing consecutive relation transformations.
Take the following query that \emph{finds all the artists who have sung songs composed by John Lennon} as an example:
\begin{equation*}
    q[A] = \exists V~\emph{Compose(John Lennon}, V) \land \emph{SungBy}(V, A)
\end{equation*}
It is embeded as
$\bsq = \mathcal{P}_{\text{SungBy}}(\mathcal{P}_{\text{Compose}}(\be_{\text{John Lennon}}))$.
Note that relation projection operation can be seen as a relation traversal from one fuzzy set of entities to another fuzzy set and may yield a huge number of results, yet here we represent it with a single fixed-size embedding, making \modelname~scalable.


% \subsection{Embedding Space}
% The essence of embedding a logical query is to represent its answer set $A$.
% We propose to embeds entities as \emph{stochastic vectors}, i.e. $\be \in $
% We propose to embed entities and queries into the same space: $\be, \bsq \in [0,1]^d$. 
% We model the 
% Using this embedding space provides the following benefits:
% (i) Each dimension of the embedding vector is between $[0,1]$, which satisfies the domain and range requirements of fuzzy logic and allows the model to execute element-wise fuzzy conjunction/disjunction/negation.
% (ii) The representation is endowed with probabilistic interpretation.
% Particularly, this domain restriction is implemented with an element-wise sigmoid function.


\section{Methodology}
In this section, we present our model \modelname, which uses fuzzy operations to implement logical operators.

\subsection{Logical query embedding}
Our objective is to design a query embedding model that can fit the axiomatic system of classical logic and retain the properties in Table \ref{tab:axioms}. 
Considering fuzzy logic systems is a natural direction, as their axiomatic systems are fully compatible with classical logic, and their logical operations therefore conform to these properties as well. 
Furthermore, fuzzy logic allows values to float between $[0,1]$, which allows us to design end-to-end differentiable logic operators as opposed to $0,1$ Boolean logic.
% A natural direction is to consider fuzzy logic systems, as their axiomatic systems are fully compatible with classical logic, and their logical operations therefore conform to these properties as well. 
In our work, we implement the logical operators in vector space through element-wise fuzzy conjunction, fuzzy disjunction and fuzzy negation.
This design ensures that we can satisfy the requirements of Table \ref{tab:axioms} in all dimensions.
Particularly, we present \modelname~with reference to product logic, one of the most prominent fuzzy logic systems \cite{KlementTNormBook}.
Alternative design choices based on \luka~and \godel~logic are discussed in Appendix \ref{ap:tnorm}.
% During training, we optimize the ranking-based objective for each dimension in order to ensure that \modelname~fulfills the properties in Table \ref{tab:axioms}.
% We optimize the ranking-based objective for each dimension during training, ensuring that for each dimension, \modelname~satisfy the above properties of logical operations.

\paragraph{Embedding Space} 
We propose to embed entities and queries into the same space: $\be, \bsq \in [0,1]^d$.
Using this embedding space provides the following benefits:
(i) Each dimension of the embedding vector is between $[0,1]$, which satisfies the domain and range requirements of fuzzy logic and allows the model to execute element-wise fuzzy conjunction/disjunction/negation.
(ii) The representation is endowed with probabilistic interpretation.
Particularly, this domain restriction is implemented with an element-wise sigmoid function.

\paragraph{Atomic Query}
We first discuss how to embed an atomic query like $\emph{Compose}(\emph{John Lennon}, V_?)$.
% , which is essentially representing the target variable $V_?$.
% Specifically, the objective is to derive a query embedding for the variable $V_?$  given the anchor entity embedding $\be_{\text{John Lennon}}$ and the relation representation of \emph{Compose}.
In our work, we associate each relation $r \in \mathcal{R}$ with a weight matrix $\mathbf{W}_r \in \mathbb{R}^{d \times d}$ and a bias vector $\mathbf{b}_r \in \mathbb{R}^d$.
Given a relation $r$ and the anchor entity embedding $\be$, we model the query embedding 
% for the target variable $V_?$ 
as the following relation transform:
\begin{equation*}
\footnotesize
    \bsq = \mathcal{P}_r(\be) = \boldsymbol{\sigma}( \mathbf{W}_r \be + \mathbf{b}_r)
\end{equation*}
where $\boldsymbol{\sigma}$ is an element-wise sigmoid function to impose the domain restriction $\bsq \in [0,1]^d$.
To avoid the rapid growth in number of parameters with the number of relations and alleviate overfitting on rare relations, we follow \cite{RGCN} and adopt \emph{basis-decomposition} to define $W_r$: 
\begin{equation*}
    \mathbf{W}_r = \sum_{i=1}^{m} a_{ri}\mathbf{M}_i
\end{equation*}
i.e. as a linear combination of $m$ basis transformations $\mathbf{M}_i \in \mathbb{R}^{d \times d}$ with coefficients $a_{ri}$ that depend on $r$. It can be seen as a form of effective weight sharing among different relation types. Note that intermediate variables can be embeded by performing multiple
such transformations.

% and \modelname~can therefore handle existential quantifier.
% Take the following query that \emph{finds all the artists who have sung songs composed by John Lennon} as an example:
% \begin{equation*}
%     q[V_?] = \exists V~\emph{Compose(John Lennon}, V) \land \emph{SungBy}(V, V_?)
% \end{equation*}
% It is embeded as
% $\bsq = \mathcal{P}_{\text{SungBy}}(\mathcal{P}_{\text{Compose}}(\be_{\text{John Lennon}}))$.

\paragraph{Existential Quantifier ($\exists$)}
A query involving existential quantified variables can be embeded by performing consecutive relation transformations.
Take the following query that \emph{finds all the artists who have sung songs composed by John Lennon} as an example:
\begin{equation*}
    q[V_?] = \exists V~\emph{Compose(John Lennon}, V) \land \emph{SungBy}(V, V_?)
\end{equation*}
It is embeded as
$\bsq = \mathcal{P}_{\text{SungBy}}(\mathcal{P}_{\text{Compose}}(\be_{\text{John Lennon}}))$.
Note that relation projection operation can be seen as a relation traversal from one fuzzy set of entities to another fuzzy set and may yield a huge number of results, yet here we represent it with a single fixed-size embedding, making \modelname~scalable.

\paragraph{Logical Connectives ($\land, \lor, \neg)$}
We propose to use fuzzy logic operations to model logic connectives in vector space.
Following product logic with \luka~negator \cite{KlementTNormBook}, the embeddings of $q_1 \land q_2$, $q_1 \lor q_2$, and $\neg q$ are computed as follows:
\begin{alignat*}{2}
        q_1 \land q_2: & \quad \conjop(\bsq_1, \bsq_2) && =   \bsq_1 \circ \bsq_2 \\
        q_1 \lor q_2: & \quad \disjop(\bsq_1, \bsq_2) && = \bsq_1 + \bsq_2 - \bsq_1 \circ \bsq_2 \\
        \neg q: & \quad \negop(\bsq) && = \mathbf{1} - \bsq
\end{alignat*}
where 
$\circ$ denotes element-wise multiplication (fuzzy conjunction),
and $\mathbf{1}$ is the all-ones vector.
$\mathcal{D}$ corresponds to product logic fuzzy disjunction $x \oplus y = x+y - xy, x,y \in [0,1]$.
% \bsq_1 \oplus \bsq_2
% $\bot: [0,1]^d \times [0,1]^d \rightarrow [0,1]^d$ and $\top: [0,1]^d \times [0,1]^d \rightarrow [0,1]^d$  denote the element-wise \tnorm~and \tconorm~respectively, and $\mathbf{1}$ is the all-ones vector.
 


\paragraph{Scoring Function}
% Given a query $q$ and an entity $e$, $\phi(q,e)$ evaluates the truth value of the FOL formula when replacing the target variable in $q$ with $e$.
% With $\be, \bsq \in [0,1]^d$, 
We estimate the plausibility that $e$ answers $q$ by dot product:
% $\phi(q, e) =  \be^\intercal \bsq$.
\begin{equation} \label{eq:scoring}
  \phi(q, e) =  \bsq^\intercal \be
    % \phi(q, e) = \text{LN}(\bsq)^\intercal \text{LN}(\be)
\end{equation}
% where $LN$ is Layer Normalization \cite{LayerNorm}.
% $\phi(q, e) = \sigma( \bsq^\intercal \be )$.
In practice, multiple conjunction operations tend to diminish the norms of query embeddings. In order to mitigate the influence of query complexity, we apply Layer Normalization \cite{LayerNorm} before computing the score.

% \begin{equation} \label{eq:scoring}
%     \phi(q, e) = \text{LN}(\bsq)^\intercal \text{LN}(\be)
% \end{equation}
% where $LN$ is Layer Normalization \cite{LayerNorm}.


\subsection{Model learning and inference}
% \paragraph{Training objective}
% Our objective is to maximize the element-wise score of a query and its answers while minimizing the element-wise score of a query and negative samples.
During training, given a query embedding $q$, we optimize the following negative log-likelihood loss:
\begin{equation*}
\footnotesize
    L = - \log \sigma (\phi(q,e) - \gamma) 
        - \sum_{j=1}^n \frac{1}{n} \log \sigma (\gamma - \phi(q,e'))
\end{equation*}
where $e$ is an entity in the answer set of $q$, $e'$ represents a random negative sample, and $\gamma$ denotes the margin. We use $n$ random negative samples and optimize over the average. 

For inference, given a query $q$, \modelname~embeds it as $\bsq$ and rank all the entities by $\phi(q, \cdot)$.




\subsection{Theoretical Analysis} \label{sec:theory}
For \modelname, we present the following propositions with proof in Appendix \ref{ap:propproof}.
\begin{proposition}
Our conjunction operator $\conjop$ is commutative, associative, and satisfies conjunction elimination. 
% \YS{double check: C appears twice}
\end{proposition}
\begin{proposition}
Our disjunction operator $\disjop$ is commutative, associative, and satisfies disjunction amplification. 
% \YS{double check: should this one be about disjuction?}
\end{proposition}
\begin{proposition}
Our negation operator $\negop$ is involutory and satisfies non-contradiction.
\end{proposition}







% \subsubsection{1-d case}
% In the one-dimensional case, we encode entity $e$ and query $q$ as real numbers in $[0,1]$: $\be, \bsq \in [0,1]$. We use the canonical negator $c(x)$ to define negation operator and \tnorm~$t(a,b)$ and \tconorm~$s(a,v)$ of Table \ref{tab:tnorms} to define the conjunction operator and the disjunction operator respectively.
% \begin{table}[h]
%     \centering
%     \begin{tabular}{rl}
%         $q_1 \land q_2$: & $t(\bsq_1, \bsq_2)$ \\
%         $q_1 \lor q_2$: & $s(\bsq_1, \bsq_2)$ \\
%         $\neg q$: & $1 - \bsq$
%     \end{tabular}
% \end{table}

% To estimate the probability that $q$ is an answer to $q$, we define the following conjunction based scoring function $\phi(v,q)$:
% \begin{equation*}
%     \phi(v, q) = t(\be, \bsq)
% \end{equation*}

% \begin{proposition}
% Our conjunction operator $\conjop$ and disjunction operator $\conjop$ are commutative, associative, and monotonic.
% \end{proposition}
% \begin{proposition}
% Our negation operator $\negop$ is involutory and monotonic.
% \end{proposition}






% \subsubsection{n-dimensional case}

% % Entities
% % - Entity initialization
% % - Query embedding process


% % Fuzzy logic requires that the function inputs and outputs must be a real number in $[0,1]$. 
% % To ensure our embedding semantics conform to the logic operations, we model entities and queries with $\bs \in [0,1]^d$.
% % % Formally, an entity set $S$ is represented by $\bs \in [0,1]^d$, with domain restriction implemented with a sigmoid function.

% % We model entities and queries with $K$-way $d$-dimensional categorical distributions, each distribution corresponding to a property of the entity.
% % In our model, we assume that each entity has a deterministic value for each property, being a one-hot categorical distribution distribution.

% % Therefore we restrict our entity embedding $\be$ and entity set embedding $\bs$ to $\be, \bs \in [0,1]^d$.
% % We consider an entity set $S$ as a property value distribution, and an entity $v \in S$ is a sample sampled from the set.
% % we encode an entity set or an entity as a vector $\Svec \in \mathbb{R}^d$, with $0 \leq v[i] \leq 1, i=1,...,d$, where each entry can be interpreted as an entity property represented by a Bernoulli distribution.


% \paragraph{Logical Operators}
% % To model logical operations in a principled and learning-free manner, we borrow the fuzzy logic operations and apply them in the vector space.
% % Here we describe the design of operators in computation graphs, which include the relation projection operator $\mathcal{P}$ and logical operators: intersection operator $\mathcal{I}$, union operator $\mathcal{U}$, and negation $\mathcal{N}$.
% % We define the logic operators with reference to the \tnorm~based fuzzy logic system.
% % As in many fuzzy set mathematical models, we use \tnorm~to model intersection and the standard negator $c(x)=1-x$ to model negation, and use the corresponding \tconorm~for union.
% We define the logical operators based on the minimum \tnorm~as follows:

% \begin{table}[h]
%     \centering
%     \begin{tabular}{ll}
%         $q_1 \land q_2$: & $\bot (\bsq_1, \bsq_2)$ \\
%         $q_1 \lor q_2$: & $\top (\bsq_1, \bsq_2)$ \\
%         $\neg q$: & $\mathbf{1} - \bsq$
%     \end{tabular}
% \end{table}

% where $\bot$ and $\top$ denote element-wise minimum and maximum respectively, and $\mathbf{1}$ is the all-ones vector.
% % Specifically, given $n$ input embeddings $\{\Svec_1, ..., \Svec_n \}$, we model the logic operator output as follows:
% The minimum \tconorm~and maximum \tconorm~are known as the \emph{standard fuzzy conjunction} and \emph{standard fuzzy disjunction}.
% Analysis about the choices of logic systems and possible alternatives are given in Appendix \ref{ap:otherlogic}.














% \subsection{Theoretical analysis}
% In this section, we provide some theoretical analyses of \modelname~and other existing approaches.
% We first discuss the expressiveness of the model for an atomic formula like $\textsl{Compose}(\text{John Lennon}, V)$, and then we discuss whether the logical operators can preserve the basic properties of those logical connectives in vector space.

% \subsubsection{Fully Expressiveness}
% In this section, we investigate the expressiveness of a logical query embedding model for an atomic formula. The key here is the definition of the set embedding of the model.

% [Query2Box: translational, not fully expressive. symmetric => reflexive]

% \subsubsection{Preserve properties of logical operations}


% % For example, Query2Box \cite{Query2Box} proposes to exploit the equivalence of logical operations and set operations in this task. 
% % Query2Box uses box to represent sets and box overlapping to represent set intersection as a way to represent logical operations.
% % BetaE \cite{BetaE} represents the set $S$ as a beta distribution $p_S=\mathcal{B}[\alpha_S, \beta_S]$ ($\alpha_S$ and $\beta_S$ are shape parameters for the beta distribution $\mathcal{B}$) and defines set intersection result as the weighted product of the input distributions:
% % $p_{S_1 \cap S_2}=\frac{1}{Z} \prod p_{S_1}^{w_1} p_{S_2}^{w_2}$, where $Z$ is a normalization constant and $w_1, w_2$ are learnable weights. In case of identical weights, the operation is equivalent to the product \tnorm.
% % In terms of complement (negation), BetaE proposes the complement operator as $p_{\overline{S}} = \mathcal{B}[\frac{1}{\alpha_S}, \frac{1}{\beta_S}]$ and proves that this operator is involutory. However, this operator does not satisfies the monotonicity requirement. [Add a figure]
% % For instance, suppose $p_S=\mathcal{B}[2,5]$, then $p_{\overline{S}} =\mathcal{B}[1/2, 1/5]$. 
% % Since $p_S(0.1)=2.0 > p_S(0.5)=0.9$, we would correspondingly expect $p_{\overline{S}} (0.1) < p_{\overline{S}} (0.5)$, while this condition does not hold because $p_{\overline{S}} (0.1)=0.5 > p_{\overline{S}} (0.5)=0.4$.
% % [replace with a figure and put it in appendix]



\begin{align*}
    \footnotesize
    q[A] 
    \triangleq ?A. & 
    \exists V_1, ..., V_k.
    (v_{11} \land ... \land v_{1m_{1}}) \lor ... \lor (v_{n1} \land ... \land v_{nm_{n}}) \\
    \text{where}& ~v_{ij} = r(e, V) 
        \text{or}~v_{ij} = \neg r(e, V)~
        \text{with}~r \in \mathcal{R}, e \in \mathcal{E}, V \in {A, V_1, ..., V_k} \\
    \text{or}& ~v_{ij} = r(V, V')~
        \text{or}~v_{ij} = \neg \neg r(V,V'),
        \text{with}~r \in \mathcal{R}, V,V' \in {A, V_1, ..., V_k}, V \neq V'
\end{align*}

% We are interested in answering first-order logic (FOL) queries with logical operations including existential quantification ($\exists$), conjunction ($\land$), disjunction($\lor$), and negation ($\neg$). 
% Note that we do not consider FOL queries with universal quantification ($\forall$) in this paper, since queries with universal quantification hardly apply in real-world KGs considering that no entity connects with all the other entities.
% An FOL query on KG consists of atomic queries, existential quantifiers, and logical connectives $\land, \lor, \neg$.

% \includegraphics[height=0.8em]{figures/musicnote.jpg} 
% (/fy\"uk/)
% (\underline{Fu}zzy \underline{Qu}ery \underline{E}mbedding)
% \footnote{``FuQuE'' (/fju:k/) imitates the word ``fugue'', a music composition.}.
% \footnote{``Fuge'' is German for the musical composition ``fugue''.}. 

Although CQD \cite{CQD} proposes to train a link prediction model (e.g. ComplEx \cite{ComplEx}) with only KG edges and generalize to complex FOL queries in the inference stage, it has significant scalability issue.
it does not provide a FOL query embedding and its inference requires ranking all the entities for each atom query, which still faces the aforementioned scalability challenge. Furthermore,  such link predictor based models cannot take advantage of complex query training samples, and its inference accuracy is thus bound by KG link prediction performance.

% , and such training data is not readily available in most of the real-world KGs.
% This draback motivates CQD \cite{CQD} to train a link prediction model (e.g. ComplEx \cite{ComplEx}) using only KG edges and generalize to complex queries through gradient-based optimization or beam search in the inference stage. 
While CQD exhibits great generalization capability on Existential Positive First-Order (EPFO) Queries, it has the following limitations: (i) CQD cannot benefit from complex query training sets, and its performance is thus limited by KG link prediction performance. (ii) Considering that real-world KGs are composed of millions of entities, the inference inefficiency greatly affects its use in practice. CQD either uses gradient descent to optimize query embedding or use beam search to search for intermediate entities. It is significantly less efficient than the aforementioned methods, such as Query2Box, which is capable of constant time inference using locality hashing. 




To address these issues, recent approaches attempt to leverage embeddings to infer missing KG facts.
The logical query embedding methods represented by GQE \cite{GQE}, Query2Box \cite{Query2Box}, BetaE \cite{BetaE} seek to embed logical queries and entities in the same vector space and conduct query answering via dense similarity search.
The key idea is to transform the query into a computation graph (Fig. \ref{fig:computation_graph}) and compute the query embedding in a bottom-up manner. Each leaf node represents an anchor entity's embedding and each edge represents a deep architecture based transformation of relation projection or logical operation.
Such approaches robustly handles missing edges and offers significant advantages in terms of time and space complexity of inference, since they do not need to track the intermediate entities and reduce this problem to dense similarity search (e.g. nearest neighbor search), which could be performed efficiently by methods like locality sensitive hashing \cite{indyk1998approximate}.
% By learning the deep architecture of the related projection or logical operation, these techniques attempt to embed the query and entity in the same space.

To address these issues, 
% In order to efficiently answer complex logical queries on KG while generalize for missing edges, 
recent works \cite{GQE, Query2Box, BetaE} seek to embed logical queries and entities in the same vector space and conduct query answering via dense similarity search.
The key idea of logical query embedding is to implement logical operation in a differentiable way and iteratively compute embedding from leaf nodes to root node according to the computation graph (Figure \ref{fig:computation_graph}).
Such approaches robustly handles missing edges and offers significant advantages in terms of time and space complexity of inference
, since they do not need to track the intermediate entities and reduce this problem to dense similarity search (e.g. nearest neighbor search), which could be performed efficiently by methods like locality sensitive hashing \cite{indyk1998approximate}.
However, the logic operators in these models are defined in an ad-hoc fashion, many of which do not satisfy the axiomatic system of classical logic or fuzzy logic \cite{KlementTNormBook}, which limits their inference accuracy. 
Furthermore, the logical operators of existing works are based on multi-layer perceptron (MLP) and/or attention mechanism, which requires a large number of training queries containing such logic operations to learn the parameters. This greatly limits the scope of application of the models,
since it is extremely challenging to collect a large number of reasonable complex queries with accurate answers, and such training data is not readily available in most of the real-world KGs.


\begin{equation*}
    \mathcal{C}(
        \mathcal{B}[\alpha_1, \beta_1],...,\mathcal{B}[\alpha_n, \beta_n]
    ) = \mathcal{B}[ \sum_{i} w_i \alpha_i, \sum_{i} w_i \beta_i]
\end{equation*}

The disadvantages are that the model cannot represent the disjunction result as a closed form with the same number of parameters, and that converting the original query to a DNF may result in an exponential increase in the number of clauses and operations.

% GQE and Query2Box does not directly define the disjunction operator. 
% GQE and Query2Box do not define the disjunction operator directly. For queries containing disjunction, the model will first convert it to its equivalent Disjunctive Normal Form (DNF) to ensure that disjunction only disjunction appears only in the last step of the computation. Based on this, the disjunction operator directly retains all input embeddings without extra computation.
% This approach was proposed by Query2Box, motivated by the fact that a union of multiple boxes is no longer a box and the disjunction can only be executed at the last step. 
% Query2Box extends GQE to have the same disjunction expressivity.
% \emph{DM} of BetaE means that it uses De Morgan's law to generate disjunction embeddings.

For the DNF rewriting method, the model first rewrites the query as a Disjunctive Normal Form (DNF) to ensure that the disjunction appears only in the last step and then directly retains all input embeddings.  

% Moreover, the conjunction operator of Query2Box is not a strict box intersection but an approximation by deep sets \cite{DeepSets}. We assume the most ideal case for Query2Box that its deep architecture can always yield the exact box intersection.

GQE does not satisfy associativity because the averaging operation is not associative: $\frac{1}{2}(\frac{1}{2}(a+b)+c) \not\equiv \frac{1}{2}(a + \frac{1}{2}(b+c))$ where $a,b,c \in \mathbb{R}$.

For example, supposing that $e$ and $q_1 \land q_2$ locate at the same point and $\bsq_1 \neq \bsq_2$, we have $\phi(q_1 \land q_2, e) > \phi(q_1 \land q_2, e)$.

% For all the three models, their original conjunction operators utilize deep architectures (e.g., deep sets \cite{DeepSets} or attention mechanism) to learn input sub-query weights to put emphasis on the potentially more important sub-query.
% Therefore, 

Note that for conjunction, we omit the sub-query weighing mechanism of these models in Table \ref{table:baseline-geo}.
For all the three models, their original conjunction operators utilize deep architectures (e.g., deep sets \cite{DeepSets} or attention mechanism) to learn input sub-query weights to put emphasis on the potentially more important sub-query.
Therefore, we assume that all input embeddings have the same weights and strip those deep transformations in our analysis. 
Moreover, the conjunction operator of Query2Box is not a strict box intersection but an approximation by deep sets \cite{DeepSets}. We assume the most ideal case for Query2Box that its deep architecture can always yield the exact box intersection.
The original conjuncti

% it is extremely costly to collect a large number of reasonable complex queries, and such training data is not available for many KGs.

% \item Our model can model arbitrary logic operations in closed form. This closure property means that logical operations can be arbitrarily combined, and the query embedding could always be computed in time linear in the number of clauses.
% \end{enumerate}

For instance, suppose $p_S=\mathcal{B}[2,5]$, then $p_{\overline{S}} =\mathcal{B}[1/2, 1/5]$. Since $p_S(0.1)=2.0 > p_S(0.5)=0.9$, we would correspondingly expect $p_{\overline{S}} (0.1) < p_{\overline{S}} (0.5)$, while this condition does not hold because $p_{\overline{S}} (0.1)=0.5 > p_{\overline{S}} (0.5)=0.4$.


Although not systematically defined, much of the existing work has been infiltrated with similar ideas from fuzzy set theory.

% \begin{equation*}
%     \text{(MP) \quad from}~\varphi~\text{and}~
%     \varphi \rightarrow \psi
%     ~\text{infer}~\psi
% \end{equation*}

Boolean Logic are defined by 
the following components \cite{chvalovsky2012independence}:
\begin{itemize}
    \item Semantics
    \begin{enumerate}
        \item Interpretation. $I: \mathcal{L} \rightarrow \{0,1\}$
        \item Implication. $\varphi \rightarrow \psi$ holds if and only if $I(\psi) \geq I(\varphi)$
    \end{enumerate}
    
    \item A deductive system
    \begin{enumerate}
        \item The Modus Ponen inference rule:
            \begin{equation*}
                \text{(MP) \quad from}~\varphi~\text{and}~
                \varphi \rightarrow \psi
                ~\text{infer}~\psi
            \end{equation*}
            
        \item A set of axioms (written in Hilbert deductive system)
    \end{enumerate}
\end{itemize}



% In order to embed logical queries for query answering, previous works \cite{GQE, Query2Box, BetaE} define logical operations in vector space as transformations of query embeddings. 
% Based on the anchor entity embeddings and these logical operators we can encode the queries in the same space as entities, and the probability that entity $v$ is the answer of query $q$ can be computed using a distance based scoring function $\phi(v, q)$.
% Appendix \ref{ap:baselineanalysis} provides a detailed discussion of prior works.




% %%%%%%%%%% FOL queries
% \begin{definition}
% (First-order logic queries).

% \paragraph{First-Order Logic Query and Computation Graph}
% % We are interested in answering first-order logic (FOL) queries on KGs. 
% % with logical operations including existential quantification ($\exists$), conjunction ($\land$), disjunction($\lor$), and negation ($\neg$). 
% % Note that we do not consider FOL queries with universal quantification ($\forall$) in this paper, since queries with universal quantification do not apply in real-world KGs considering that no entity connects with all the other entities.
% A first-order logic query $q$ involve existential quantification ($\exists$), conjunction ($\land$), disjunction($\lor$), and negation ($\neg$). It consists of a single target variable $V_?$ which provides query answers, a number of \emph{anchor entities} from the KG, and optionally some existentially quantified bound variables.
% % $V_1, ..., V_k \subseteq \mathcal{V}$ for intermediate results.
% % Formally, the disjunctive normal form (DNF) of a query $q$ can be written as follows:
% % \begin{equation*}
% %     q[V_?] = V_?. \exists V_1, ..., V_k: C_1 \lor C_2 \lor ... \lor C_n
% % \end{equation*}
% % where each $C$ represents a conjunctive clause with one or more literals, and each literal represents an atomic formula or its negation.
% % \begin{enumerate}
% %     \item Each $C$ represents a conjunctive query with one or more literals $e$. $C_i = e_{i1} \land e_{i2} \land ... \land e_{im}$
% %     \item Each literal $e$ represents an atomic formula (triple) or its negation. $e_{ij}=r(v_a, E)$ \text{or} $\neg r(e_a, V)$ \text{or} $r(V',V)$ \text{or} $\neg r (V', V)$, where $v_a \in \mathcal{V}_a, V \in \{V_?, V_1, ..., V_K\}, V' \in \{V_1, ..., V_K\}, V \neq V', r \in \mathcal{R}.$
% % \end{enumerate} 
% %%%%%%%%%% Computation Graph
% As shown in Fig. \ref{fig:computation_graph}, the \emph{computation graph} \cite{GQE} of a query 
% % $q$ as the graph with edges formed between the anchor nodes $v_1, v_2, ...$ and the variable nodes $V_?, V_1, ..., V_m$, which 
% specifies the steps needed to compute a query.
% % and can be viewed as a heterogeneous tree 
% %  In the computation graph, 
%  Each leaf node represents an anchor entity. The internal nodes correspond to the bound variables, and the root node represents the unique target variable, i.e., the query.
% Each edge represents one of the following operations: (i) relation projection $\mathcal{P}$; (ii) conjunction $\conjop$; (iii) disjunction $\disjop$; (iv) negation $\negop$.
% % \begin{enumerate}
% %     \item Relation Projection: Given a set of entities $S \in \mathcal{V}$ and relation type $r \in \mathcal{R}$, compute adjacent entities $\bigcup_{v \in S} A_r(v)$ related to $S$ via $r$: $A_r(v) \equiv \{ v' \in \mathcal{V}: r(v, v')=\text{True} \}$.
    
% %     \item Set Intersection (Conjunction): Given sets of entities ${S_1, S_2, ..., S_n}$, compute their intersection $\bigcap_{i=1}^n S_i$.
    
% %     \item Set Union (Disjunction): Given sets of entities ${S_1, S_2, ..., S_n}$, compute their union $\bigcup_{i=1}^n S_i$.
    
% %     \item Set Complement (Negation): Given a set of entities $S \subseteq \mathcal{E}$, compute its complement $\overline{S} \equiv \mathcal{V}\setminus S$.
% % \end{enumerate}
% % To answer a given FOL query, we follow the computation graph, execute logical operators, and obtain the answers by retrieving entities in the root node.
% % We denote the answer set of query $q$ as $\llbracket q \rrbracket$.
% % The symbolic traversal of the computation graph is equivalent to traversing the KG. However, it cannot handle noisy or missing edges in the KG.
% % In order to efficiently perform complex logical queries on KG while generalizing for missing edges, recent works embed entity and query embedding in the same embedding space and define MLP and attention based logic operations \cite{GQE, Query2Box, BetaE}.


% \paragraph{Fuzzy Logic} \label{sec:fuzzyset}
% % In our work, we borrow the idea of fuzzy logic and use fuzzy conjunction, fuzzy disjunction, and fuzzy negation to define logical operators in vector space.
% % In preliminaries, we introduce the \tnorms~for set intersection and the corresponding \tconorms~for~set union.
% % In this section, we introduce representative fuzzy logic operations and their properties, and compare them with logical operators defined existing approaches.
% % Since previous works \cite{Query2Box, BetaE} mainly describe the logical operations from the perspective of set operations, we also present our theory from the perspective of fuzzy set theory to facilitate understanding and comparison. Fuzzy conjunction, disjunction, and negation in fuzzy logic correspond to fuzzy intersection, union, and complement of fuzzy sets respectively.
% % As their mathematical equivalence has been discussed in \cite{fuzzysetAxioms}, we will not distinguish between these terms in our paper.
% % Fuzzy operations are characterized by a series of properly justified axioms. Details about the axiomatic system are given in Appendix \ref{sec:fuzzyaxioms}.

% In fuzzy logic, the \luka~negation $c(x)=1-x$ is also called the \emph{canonical negator}. Functions that qualify as fuzzy conjunction and fuzzy disjunction are usually referred to in literature as \tnorms~ (triangular norms) and \tconorms~ (triangular conorms) respectively \cite{KlirFuzzyBook}.

% % \tconorm~is the logical dual form of the \tnorm, usually derived by via De Morgan's law and a negator. The details are given below.
% % \paragraph{Negator for complement}
% % The axioms of complement usually require that the complement function $c: [0,1] \rightarrow [0,1]$ should be continuous, monotonically decreasing, involutory ( $i.e. c(c(x))=x$), and satisfy the boundary conditions $c(0)=1$ and $c(1)=0$.
% % A widely accepted negator, also known as the \emph{canonical negator}, is defined as:
% % \begin{equation*}
% %     c(x) = 1-x
% % \end{equation*}

% % \paragraph{\tnorm~for intersection}
% A \tnorm~\cite{tnorm} is a function $t: [0, 1] \times [0, 1] \rightarrow [0, 1]$ which is commutative and associative and satisfies the boundary condition $t(a, 1) = a$ as well as monotonicity, i.e. $t(a, b) \leq t(c, d)$ if $a \leq c$ and $b \leq d$.
% Prominent examples of \tnorms~include minimum, product, and \luka~\tnorm. 
% % Any other continuous \tnorm~can be described as an ordinal sum of these three basic ones \cite{KlementTNormBook}.
% Their formulas and special properties are listed in Table \ref{tab:tnorms}.

% % \paragraph{\tconorm~for union}
% \tconorm~is the logical dual form of the \tnorm. Following De Morgan's law, given the canonical negator $c(x)=1-x$, the \tconorm~ $s$ of a \tnorm~$t$ is defined as
% $s(a,b) =  1 - t(1-a, 1-b)$.
% % $s(a,b) = c(t(c(a), c(b))) = 1 - t(1-a, 1-b)$.
Boolean Logic are defined by the following components \cite{chvalovsky2012independence}:
\begin{itemize}
    \item Semantics
    \begin{enumerate}
        \item Interpretation. $I: \mathcal{L} \rightarrow \{0,1\}$
        \item Implication. $\varphi \rightarrow \psi$ holds if and only if $I(\psi) \geq I(\varphi)$
    \end{enumerate}
    
    \item A deductive system
    \begin{enumerate}
        \item The Modus Ponen inference rule:
            \begin{equation*}
                \text{(MP) \quad from}~\varphi~\text{and}~
                \varphi \rightarrow \psi
                ~\text{infer}~\psi
            \end{equation*}
            
        \item A set of axioms (written in Hilbert deductive system)
    \end{enumerate}
\end{itemize}


% A \tconorm~is commutative and associative, and satisfies the boundary condition $s(a, 0) = a$ as well as monotonicity: $s(a, b) \leq s(c, d)$ if $a \leq c$ and $b \leq d$. Interested readers are referred to \cite{KlirFuzzyBook} for proofs.
% % \citet{tconormnegator} used the canonical negator $c(x)=1-x$ to define the \tconorm~ $s$ of a \tnorm~$t$ as
% % With the canonical negator $c$, the \tconorm~ $s$ of a \tnorm~$t$ is defined as
% % $s(a,b) = c(t(c(a), c(b))) = 1 - t(1-a, 1-b)$.
% The formulas of \tconorms~that correspond to the minimum, product, and \luka~\tnorms~are given in Table \ref{tab:tnorms}.

% % Among the three basic \tnorms~and \tconorms, the most commonly used one is the minimum operator \tnorm~and the maximum operator \tconorm.
% % They are also called \emph{standard fuzzy intersection} and \emph{standard fuzzy union}.
% % When applied to fuzzy sets, the standard fuzzy intersection produces the largest output of any~\tnorms, and the standard fuzzy union produces the smallest output of any~\tconorms~\cite{KlirFuzzyBook}. These features of the standard fuzzy intersection and union are significant because they both prevent the compounding of errors in the operands \cite{KlirFuzzyBook}.
% % Therefore, in our work, we focus on standard fuzzy intersection and union, while we also include the other two systems for comparison.
% % Note that the minimum \tnorm~was proposed for fuzzy set intersection by \citet{zadeh1965fuzzyset} in \citeyear{zadeh1965fuzzyset}, while the form was first studied by \godel~for fuzzy logic in 1932. We follow \cite{fuzzyimplicationbook} and refer to it \tnorm~as \godel~\tnorm.

% % \paragraph{Connection with query embedding works}
% % Although not systematically defined, much of the existing work has been infiltrated with similar ideas from fuzzy set theory.
% % [Add a table]



(iii) Conjunction elimination 
$\phi(q_1, e) \geq \phi(q_1, e')$, 
$\phi(q_2, e) \geq \phi(q_2, e')$
$\Rightarrow \phi(q_1 \land q_2, e) \geq \phi(q_1 \land q_2, e')$\\
$\phi(q_1, e) \geq \phi(q_1, e')$, 
$\phi(q_2, e) \geq \phi(q_2, e')$
$\Rightarrow \phi(q_1 \lor q_2, e) \geq \phi(q_1 \lor q_2, e')$
\begin{proof}
When $d=1$, i.e. $\bsq_1, \bsq_2, \be, \be' \in [0,1]$.\\
We first prove monotonicity for conjunction.$\conjop(\bsq_1, \bsq_2) = t(\bsq_1, \bsq_2)$. \\
If
\begin{align*}
    \phi(q_1, e) \geq \phi(q_1, e'),  \\
    \phi(q_2, e) \geq \phi(q_2, e')
\end{align*}
Then
\begin{align*}
    t(\bsq_1, \be) \geq t(\bsq_1, \be'),  \\
    t(\bsq_2, \be) \geq t(\bsq_2, \be')
\end{align*}
We accordingly have
\begin{align*}
\phi(q_1 \land q_2, e) 
    & = t(\be, \conjop(\bsq_1, \bsq_2)) \\
    & = t(\be, t(\bsq_1, \bsq_2)) \\
    & \geq t(\be', t(\bsq_1, \bsq_2)) \\
    & =\phi(q_1 \land q_2, e')
\end{align*}

When $d>1$, \modelname~enforces the digit-wise montonicity, i.e. $t(\be_i, t(\bsq_{1,i}, \bsq_{2,i})) \geq t(\be'_i, t(\bsq_{1,i}, \bsq_{2,i}))$. 
Given Eq (\ref{eq:scoring}), we have $\phi(q_1 \land q_2, e) \geq \phi(q_1 \land q_2, e')$.

Monotonicity for disjunction operator can be similarly proved.
\end{proof}


\begin{align*}
        q_1 \land q_2: & \quad \conjop(\bsq_1, \bsq_2) =   \bot (\bsq_1, \bsq_2) \\
        q_1 \lor q_2: & \quad \disjop(\bsq_1, \bsq_2) = \top (\bsq_1, \bsq_2) \\
        \neg q: & \quad \negop(\bsq) = \mathbf{1} - \bsq
\end{align*}
where $\bot: [0,1]^d \times [0,1]^d \rightarrow [0,1]^d$ and $\top: [0,1]^d \times [0,1]^d \rightarrow [0,1]^d$  denote the element-wise \tnorm~and \tconorm~respectively, and $\mathbf{1}$ is the all-ones vector.

% \citet{tconormnegator} used the canonical negator $c(x)=1-x$ to define the \tconorm~ $s$ of a \tnorm~$t$ as
% With the canonical negator $c$, the \tconorm~ $s$ of a \tnorm~$t$ is defined as
% $s(a,b) = c(t(c(a), c(b))) = 1 - t(1-a, 1-b)$.


\begin{table}[t]
\footnotesize
\centering
\caption{Basic properties of conjunction $\land$, disjunction $\lor$, and negation $\neg$ that a logical query embedding model is supposed to possess.
$\bsq_1 \conjop \bsq_2$, $\bsq_1 \disjop \bsq_2$, $\negop \bsq \in [0,1]^d$ denote the embedding of $q_1 \land q_2$, $q_1 \lor q_2$, and $\neg q$ respectively.
% $\conjop, \disjop$ denote the conjunction operator and disjunction operator respectively, which take input query embeddings and output embeddings that represent $q_1 \land q_2$ and $q_1 \lor q_2$ respectively.
$\phi:[0,1]^d \times [0,1]^d \rightarrow [0,1]$ is a scoring function that predicts the probability that entity $v$ is an answer to query $q$.}
\begin{tabular}{lll}
\toprule
\multirow{5}{*}{$\land$} 
& Commutativity &
$ \bsq_1 \conjop \bsq_2 \equiv \bsq_2 \conjop \bsq_1 $ \\
\cmidrule(lr){2-3}
& Associativitiy &
$(\bsq_1 \conjop \bsq_2) \conjop  \bsq_3 \equiv \bsq_1 \conjop (\bsq_2 \conjop \bsq_3) $  \\
\cmidrule(lr){2-3}
& Monotonicity &
% & & $t( \phi(\be, \bsq_1), \phi(\be, \bsq_2)) \leq t( \phi(\be', \bsq_1), \phi(\be', \bsq_2)) $\\
 $\phi(\be, \bsq_1) \geq \phi(\be', \bsq_1)$, \\
 & & $\phi(\be, \bsq_2) \geq \phi(\be', \bsq_2)$\\
& & $\Rightarrow \phi(\be, \bsq_1 \land \bsq_2) \geq \phi(\be', \bsq_1 \land \bsq_2)$\\
\cmidrule(lr){2-3}
& Archimedean & $\phi(\be, \bsq_1 \conjop \bsq_2) \leq \phi(\be, \bsq_1) $\\
& property & $\phi(\be, \bsq_1 \conjop \bsq_2) \leq \phi(\be, \bsq_2) $\\
% & &$\phi(v, q_1 \land q_2) \geq \phi(v', q_1 \land q_2) $ if $\phi(v, q_1) \geq \phi(v', q_1)$ and $\phi(v, q_2) \geq \phi(v', q_2)$\\

\midrule
\multirow{3}{*}{$\lor$}
& Commutativity &
$ \bsq_1 \disjop \bsq_2 \equiv \bsq_2 \disjop \bsq_1 $ \\
\cmidrule(lr){2-3}
& Associativitiy &
$(\bsq_1 \disjop \bsq_2) \disjop  \bsq_3 \equiv \bsq_1 \disjop (\bsq_2 \disjop \bsq_3) $  \\
\cmidrule(lr){2-3}
& Monotonicity 
& if $\phi(\be, \bsq_1) \geq \phi(\be', \bsq_1)$, \\
& & \quad $\phi(\be, \bsq_2) \geq \phi(\be', \bsq_2)$\\
& &
$\Rightarrow \phi(\be, \bsq_1 \lor \bsq_2) \geq \phi(\be', \bsq_1 \lor \bsq_2)$\\
\cmidrule(lr){2-3}
& Archimedean & $\phi(\be, \bsq_1 \conjop \bsq_2) \leq \phi(\be, \bsq_1) $\\
& property & $\phi(\be, \bsq_1 \conjop \bsq_2) \leq \phi(\be, \bsq_2) $\\
\midrule
\multirow{2}{*}{$\neg$}
& Involution &
$\negop(\negop \bsq ) \equiv \bsq$ \\
\cmidrule(lr){2-3}
& Monotonocity
& $\phi(\be, \bsq) \geq \phi(\be', \bsq)$\\
& & $\Rightarrow \phi(\be, \neg \bsq) \leq \phi(\be', \neg \bsq) $\\
\bottomrule
\end{tabular}
\label{tab:properties}
\end{table}



% Our objective is to maximize the score of the embedding of a query and its answers while minimizing the score of a query and negative samples.

% FOL queries consist of atomic formulas such as $\textsl{Compose}(\text{John Lennon}, V)$ and logical connectives like $\land$.
% We model logical operators in vector space using fuzzy logic operations.
% To make our embedding semantics conform to the logic system operations, we consider an entity as having $N$ properties, each property modeled by a $k$-dimensional categorical distribution. Relations are modeled as distribution transformations.

% We consider the relation as a transformation from one distribution to another.
% The goal here is that for all entities covered by the input distribution, we can derive the embedding distribution that covers entities in projection results.
% Specifically, 

We propose to embed logical queries by modeling logical operations with fuzzy logic functions.
We first discuss the one-dimensional case of our model and show that such modeling can fully satisfy the properties in Table \ref{tab:properties}, and then we generalize to the n-dimensional case.

Notation wise, we use boldfaced letters $\be$ and $\bsq$ to represent the embedding of  entity $v$ and query $q$ respectively.

\subsubsection{1-d case}
In the one-dimensional case, we encode entity $e$ and query $q$ as real numbers in $[0,1]$: $\be, \bsq \in [0,1]$. We use the canonical negator $c(x)$ to define negation operator and \tnorm~$t(a,b)$ and \tconorm~$s(a,v)$ of Table \ref{tab:tnorms} to define the conjunction operator and the disjunction operator respectively.
\begin{table}[h]
    \centering
    \begin{tabular}{rl}
        $q_1 \land q_2$: & $t(\bsq_1, \bsq_2)$ \\
        $q_1 \lor q_2$: & $s(\bsq_1, \bsq_2)$ \\
        $\neg q$: & $1 - \bsq$
    \end{tabular}
\end{table}

To estimate the probability that $q$ is an answer to $q$, we define the following conjunction based scoring function $\phi(v,q)$:
\begin{equation*}
    \phi(v, q) = t(\be, \bsq)
\end{equation*}

\begin{proposition}
Our conjunction operator $\conjop$ and disjunction operator $\conjop$ are commutative, associative, and monotonic.
\end{proposition}
\begin{proposition}
Our negation operator $\negop$ is involutory and monotonic.
\end{proposition}






\subsubsection{n-dimensional case}
\paragraph{Entity and query embedding}
We propose to embed entities and queries into the same space: $\be, \bsq \in [0,1]^d$ with $\norm{\be}=\norm{\bsq}= 1$.
Using this embedding space provides the following benefits:
(i) Each dimension of the embedding vector is between $[0,1]$, which satisfies the domain and range requirements of fuzzy logic operations, which allows us to perform element-wise fuzzy logic operations.
(ii) The representation is endowed with probabilistic interpretation.



\subsubsection{1-d case}
In the one-dimensional case, we encode entity $e$ and query $q$ as real numbers in $[0,1]$: $\be, \bsq \in [0,1]$. We use the canonical negator $c(x)$ to define negation operator and \tnorm~$t(a,b)$ and \tconorm~$s(a,v)$ of Table \ref{tab:tnorms} to define the conjunction operator and the disjunction operator respectively.
\begin{table}[h]
    \centering
    \begin{tabular}{rl}
        $q_1 \land q_2$: & $t(\bsq_1, \bsq_2)$ \\
        $q_1 \lor q_2$: & $s(\bsq_1, \bsq_2)$ \\
        $\neg q$: & $1 - \bsq$
    \end{tabular}
\end{table}

To estimate the probability that $q$ is an answer to $q$, we define the following conjunction based scoring function $\phi(v,q)$:
\begin{equation*}
    \phi(v, q) = t(\be, \bsq)
\end{equation*}

\begin{proposition}
Our conjunction operator $\conjop$ and disjunction operator $\conjop$ are commutative, associative, and monotonic.
\end{proposition}
\begin{proposition}
Our negation operator $\negop$ is involutory and monotonic.
\end{proposition}




\begin{table*}[t]
\centering
\caption{Basic properties of logic operations that a logical query embedding model is supposed to possess. $\phi(v, q)$ is a scoring function that estimates the plausibility that entity $v$ is an answer to query $q$.}
\begin{tabular}{lll}
\toprule
\multirow{3}{*}{conjunction} 
& commutativity &
$\phi(v, q_1 \land q_2) = \phi(v, q_2 \land q_1)$ \\
& associativitiy &
$\phi(v, q_1 \land q_2 \land q_3) = \phi(v, q_1 \land (q_2 \land q_3))$ \\
& monotonicity & 
$\phi(v, q_1 \land q_2) \geq \phi(v', q_1 \land q_2) $ if $\phi(v, q_1) \geq \phi(v', q_1)$ and $\phi(v, q_2) \geq \phi(v', q_2)$\\
\midrule
\multirow{3}{*}{disjunction}
& commutativity &
$\phi(v, q_1 \lor q_2) = \phi(v, q_2 \lor q_1)$ \\
& associativitiy &
$\phi(v, q_1 \lor q_2 \lor q_3) = \phi(v, q_1 \lor (q_2 \lor q_3))$ \\
& monotonicity & 
$\phi(v, q_1 \lor q_2) \geq \phi(v', q_1 \lor q_2) $ if $\phi(v, q_1) \geq \phi(v', q_1)$ and $\phi(v, q_2) \geq \phi(v', q_2)$\\
\midrule
\multirow{2}{*}{negation}
& involution &
$\phi(v, q) = \phi(v, \neg (\neg q))$ \\
& monotonocity &
$\phi(v, \neg q) \leq \phi(v', \neg q) $ if $\phi(v, q) \geq \phi(v', q)$\\
\bottomrule
\end{tabular}
\label{tab:properties}
\end{table*}



Based on the three \tnorms~listed in Table 1, we define the three sets of intersection and union operators, namely \godel, product, and \luka~logic as follows:


\paragraph{Scoring function}
Given an entity embedding $\be$ and a query embedding $\bsq$, 
we define the probability that $v$ is an answer of $q$ as $\score{e}{q}=\frac{\be^\intercal \bsq}{\Vert \be \Vert \Vert \bsq \Vert}$.
% \begin{equation}
%     \score{e}{q} 
%         = P(q | e)
%         = \frac{P(e|q)P(S)}{P(e)}
%         = \frac{\be^\intercal \bsq}{\Vert \be \Vert \Vert \bsq \Vert}
% \end{equation}


\paragraph{Learning objective}
Our objective is to maximize the score of the embedding of a query and its answers while minimizing the score of a query and negative samples.
The training objective is defined as follows:
\begin{equation}
    L = - \log \sigma(\score{e}{q} - \gamma) 
        - \sum_{j=1}^n \frac{1}{n} \log \sigma (\gamma - \score{e'}{q})
\end{equation}
where $e$ belongs to the answer set of $q$, $e'$ represents a random negative sample, and $\gamma$ denotes the margin. We use $n$ random negative samples and optimize over the average.



We model entities and queries with $K$-way $d$-dimensional categorical distributions, each distribution corresponding to a property of the entity.
In our model, we assume that each entity has a deterministic value for each property, being a one-hot categorical distribution distribution.


Fuzzy logic requires that the function inputs and outputs must be a real number in $[0,1]$. 
To ensure our embedding semantics conform to the logic operations, we model entities and entity sets with Bernoulli distributions.
Formally, an entity set $S$ is represented by $\bs \in [0,1]^d$, with domain restriction implemented with a sigmoid function.
An entity $v \in S$ is considered a sample sampled from the set with $\be \in \{0,1\}^d$, which are learned by the Gumbel-Softmax reparameterization trick from \cite{GumbelSoftmax}.
We provide a theoretical analysis in Appendix \ref{ap:analysis} and prove that such modeling preserves the basic properties of logical operators.

In practice, since discrete representations of entities are naturally difficult to learn, we relax the restriction and explore representing entities by Bernoulli distributions as well. 
We employee continuous representations by default, and the variant that adopts discrete representations for entities is specially denoted as \modelname$_{01}$.


Given an entity embedding $e$ and a query embedding $q$, we define the membership score as the following posterior probability:
\begin{equation}
    \score{e}{q} 
        = P(q | e)
        = \frac{P(e|q)P(S)}{P(e)}
        = \frac{\be^\intercal \bsq}{\Vert \be \Vert \Vert \bsq \Vert}
\end{equation}


\begin{align*}
   \text{\godel:}  & \mathcal{I}(\Svec_1, \Svec_2)=\text{MIN}(\Svec_1, \Svec_2) \\
    & \mathcal{U}(\Svec_1, \Svec_2)=\text{MAX}(\Svec_1, \Svec_2) \\
   \text{Product:}  & \mathcal{I}(\Svec_1, \Svec_2)=\Svec_1 \circ \Svec_2 \\
    & \mathcal{U}(\Svec_1, \Svec_2)=\Svec_1+\Svec_2 - \Svec_1 \circ \Svec_2\\
   \text{\luka:}  & \mathcal{I}(\Svec_1, \Svec_2)=\text{MAX}(\Svec_1+\Svec_2-1, 0)\\
    & \mathcal{U}(\Svec_1, \Svec_2)=\text{MIN}(\Svec_1+\Svec_2-1, 1)
\end{align*}
where $\circ$ is the element-wise product, and \text{MAX} and \text{MIN} denote element-wise maximum and minimum respectively.

% Therefore we restrict our entity embedding $\be$ and entity set embedding $\bs$ to $\be, \bs \in [0,1]^d$.
We consider an entity set $S$ as a property value distribution, and an entity $v \in S$ is a sample sampled from the set.
we encode an entity set or an entity as a vector $\Svec \in \mathbb{R}^d$, with $0 \leq v[i] \leq 1, i=1,...,d$, where each entry can be interpreted as an entity property represented by a Bernoulli distribution.


To address the above issues, we present \modelname~
\includegraphics[height=0.8em]{figures/musicnote.jpg} 
(/fy\"uk/)
(\underline{Fu}zzy \underline{Logic} based \underline{Qu}ery \underline{E}mbedding)
\footnote{``FuQuE'' (/fju:k/) imitates the word ``fugue'', a music composition.}.


% conclusion
The results are encouraging and suggest various extensions, including different fuzzy logic systems as well as deeper transformation architectures for relation projection. Another direction is to use the defined logical operators to incorporate logical rules to further enhance reasoning on KGs. Furthermore, we are also interested in jointly learning embeddings for logical queries and natural language questions to enhance question answering on KGs.

%  The function $t$ define a general class of intersection operators for fuzzy sets, for which we refer to \cite{fuzzyimplicationbook} for proofs.

We use lower-letter script (e.g. $v_i$) for a single entity and upper-case script (e.g. $V_i$) to represent variables whose domain is the set of entities.

A first-order logic query $q$ consists of a single target variable $V_?$ that provides query answers, a number of anchor entities, and optionally existentially quantified bound variables $V_1, ..., V_k \subseteq \mathcal{V}$. Formally, the disjunctive normal form (DNF) of $q$ can be written as follows:
\begin{equation*}
    q[V_?] = V_?. \exists V_1, ..., V_k: C_1 \lor C_2 \lor ... \lor C_n
\end{equation*}
\begin{enumerate}
    \item Each $C$ represents a conjunctive query with one or more literals $e$. $C_i = e_{i1} \land e_{i2} \land ... \land e_{im}$
    \item Each literal $e$ represents an atomic formula (triple) or its negation. $e_{ij}=r(v_a, E)$ \text{or} $\neg r(e_a, V)$ \text{or} $r(V',V)$ \text{or} $\neg r (V', V)$, where $v_a \in \mathcal{V}_a, V \in \{V_?, V_1, ..., V_K\}, V' \in \{V_1, ..., V_K\}, V \neq V', r \in \mathcal{R}.$
\end{enumerate} 


A first-order logic query $q$ consists of a single target variable $V_?$ that corresponds to query answer, a number of existentially quantified bound variables $V_1, ..., V_k \subseteq \mathcal{V}$, a non-variable anchor entity set $\mathcal{V}_a \subseteq \mathcal{V}$. Formally, the disjunctive normal form (DNF) of $q$ can be written as follows:

% The core problem of query embedding is how to characterize entity sets. 

% The core problem of query embedding is how to characterize entity sets. 
% In our work, we consider an entity set as a fuzzy set and encode it as a vector $\Svec \in \mathbb{R}^d$, with $0 \leq \Svec[i] \leq 1, i=1,...,d$.
% In the special case of $d=|\mathcal{V}|$ (the number of entities in KG), $\Svec[i]$ can be interpreted as the degree to which entity $i$ belongs to the set, that is, the membership score of entity $i$ to the fuzzy set.
% In practice, $d$ is usually much smaller than $|\mathcal{V}|$, and we regard $\Svec$ as a sketch of the the membership score vector in the low-dimension space.
% Accordingly, each entity is regarded a set of only one element, and thus embeded as a vector $\Evec \in \mathbb{R}^d$ with $0 \leq \Evec[i] \leq 1, i=1,...,d$, to which we add a regularization term to force it to be sparse.


In this section, we first define our conjunction, disjunction, and negation operator, which are defined based on fuzzy intersection, union, and complement.

Here we describe the design of operators in computation graphs, which include the relation projection operator $\mathcal{P}$ and logical operators: intersection operator $\mathcal{I}$, union operator $\mathcal{U}$, and negation $\mathcal{N}$.

% To answer queries in a large and incomplete KG, we introduce our model \modelname, which embeds both entities and queries as distributions. We first describe our entity. define the relation projection operator, and then the intersection, union, and negation operator following the fuzzy logic connectives. Finally, we describe our training objective.

% Since previous works describe the logical operations from the perspective of set operations \cite{Query2Box, BetaE}, for the reader's understanding and comparison, we also exploit the equivalence between fuzzy logic and fuzzy set and present our work from the perspective of fuzzy set theory to be consistent.
% Their equivalence was discussed in \cite{fuzzysetAxioms} paper, and will not be distinguished in this paper.

% The fuzzy operations based on the minimum operator are called \emph{standard fuzzy operations}. 

Note that the minimum \tnorm~was proposed for fuzzy set intersection by \citet{zadeh1965fuzzyset} in \citeyear{zadeh1965fuzzyset}, while the form was first studied by \godel~for fuzzy logic in 1932. We follow \cite{fuzzyimplicationbook} and refer to it \tnorm~as \godel~\tnorm.

 The function $t$ define a general class of intersection operators for fuzzy sets, for which we refer to \cite{fuzzyimplicationbook} for proofs.
 
 The fuzzy operations based on the minimum operator are called \emph{standard fuzzy operations}.
 
 Corresponding to the class of intersection operators, a general class of union operators are called \tconorm s (triangular conorms).


Since the design of our method does not behold parameters for the logical operations to learn, it is able to achieve comparable results even when trained only with the KG edges. Furthermore, experiments show that our model outperforms previous methods when only trained with the KG edges.

Extensive experiments on two benchmark datasets demonstrate that our model not only provides state-of-the-art performance using the same training data, but also achieves comparable results to baselines even when we only use KG edges for training.

In our work, we consider all non-anchored nodes in the computational graph as fuzzy sets and define the logical operators according to fuzzy set theory.
In preliminaries, we introduce the \tnorms~for set intersection and the corresponding \tconorms~for~set union.


% Moreover, although queries could be in principle answered by directly traversing the KG, this is problematic in practice since multi-hop reasoning involves an exponential growth in computational time/space.  


% In essence, it involves answering first-order logic (FOL) queries over KGs using existential quantification ($\exists$), conjunction ($\land$), disjunction ($\lor$), and negation ($\neg$).
% An example of a FOL query is
% \begin{align*}
%     V_?:\text{Awarded}(V_?, \text{Academy Award for Best Actor)} \land \text{Awarded}(V_?, \text{Golden Globe for the Best Actor})
% \end{align*}
% which corresponds to the question ``Who have won both Academy Award for Best Actor and Golden Globe for Best Actres''.
% An example of a FOL query is for the question ``Which artists other than the Beatles Paul McCartney and John Lennon have written songs for?'', which can be written as:
% It can be used to answer questions such as  or ``Which artists other than the Beatles Paul McCartney and John Lennon have written songs for?'' \YS{``''; }


Our approach has the following major advantages compared to existing approaches:
\begin{enumerate}
\item Our method employs differentiable logical operators that fully satisfy the axioms of  logical operations and is capable of preserving logical properties in vector space. 
This makes \modelname~significantly superior to the state-of-the-art methods for answering FOL queries.
This is corroborated by extensive experiments on three benchmark datasets, which demonstrate that \modelname~delivers significantly better performance to the state-of-the-art methods in answering FOL queries.

\item Our logical operations preserve the property of the logical operations while they do not require learning any operator specific parameters. Accordingly, experimental results show that even when our model is trained on KG edges only, it achieves results comparable with state-of-the-art models that are trained with extra complex query data. Furthermore, when no complex query data is used for training, our model significantly outperforms previous models.
This is a huge advantage in real-world applications, since it is extremely costly to collect a large number of reasonable complex queries, and such training data is not available for many KGs.

% \item Our model can model arbitrary logic operations in closed form. This closure property means that logical operations can be arbitrarily combined, and the query embedding could always be computed in time linear in the number of clauses.
\end{enumerate}


[simplify and add descriptions about our model] A first-order logical query can be represented as a Directed Acyclic Graph (DAG) which specifies the steps needed to derive the answers. This DAG is called the \emph{dependency graph} or \emph{computation graph} of this query \cite{GQE}.
Consider the question ``Who won the Academy Award for Best Actor and  Golden Globe for Best Actor''. This question can be expressed in FOL as a conjunctive query:
\begin{equation*}
    V_?:\text{Awarded}(V_?, \text{Academy Award for Best Actor)} \land \text{Awarded}(V_?, \text{Golden Globe for the Best Actor})
\end{equation*}
where $V_?$ represents the target entities that we want to retrieve.
The corresponding computation graph is shown in Figure [Add figure].
To answer this query, one first locates the \emph{anchor entities} (i.e. constants in the query) \emph{Academy Award for Best actor} and \emph{Golden Globe for Best actor} in the KG.
By traversing KG by the relation ``Awarded'', one retrieves the sets of actors who won the Academy Award and Golden Globe award respectively, and then takes the intersection of these two sets to get the set of answer entities to this query. 
If we want to find the singers that Paul McCartney and Lennon wrote songs and gave away to, this query can be represented in FOL as
\begin{align*}
    V_?: \exists V 
    & (\text{ComposedBy}(V, \text{John Lennon}) \lor \text{ComposedBy}(V, \text{Paul McCartney})) \\
    & \land \neg \text{ReleasedBy}(V, \text{the Beatles}) \land \text{SungBy}(V, V_?)
\end{align*}
Similar to the previous ones, one traverses the KG and finds the songs composed by John Lennon and the songs composed by Paul McCartney respectively, takes the union of these two sets, and then finds all songs released by the Beatles, and compute the complement.
Similar to the previous one, one first finds all the songs written by Paul McCartney and all the songs written by John Lennon separately, taking a union of the two sets, and then finds all the songs released by the Beatles and compute the complement as results for $V$. Finally, one again traverses KG and finds the musicians of these songs as the answer set of this query
[figure]



% The key idea of logical query embedding is to design logical operators based on multi-layer perceptron (MLP) and attention mechanism, and embed the query into a geometric object or a parameterized probability distribution following the computation graph.

% In essence, it involves answering first-order logic (FOL) queries over KGs using existential quantification ($\exists$), conjunction ($\land$), disjunction ($\lor$), and negation ($\neg$).

% and answering an arbitrary logical query is reduced to identifying entities nearest to the embedding of the query in the vector space \cite{indyk1998approximate}.



% Existing complex query datasets are prepared by sampling on KG and collecting answers through KG traverse, and such training data are inherently affected by KG incompleteness and noise.

% The above chalenges KGs prompts the use of embedding, which represent KG entities and queries jointly in the embedding space and therefore support generalization and faster computation in KG inference 
% Such approach robustly handles missing relations and is also orders of magnitude faster, as answering an arbitrary logical query is reduced to identifying entities nearest to the embedding of the query in the vector space.
% [limitation in previous works]
% Previous methods \cite{TransE, ComplEx, RotatE, TuckER} aim to address the above challenges by using embeddings to impute the missing edges. Methods also embed logical queries into various geometric shapes in the vector space \cite{GQE, Query2Box, BetaE}.  
% The idea here is to model queries and entities as various geometric shapes, design neural logical operators and embed queries iteratively by executing logical operations according to the query computation graph. 

% An advantage of these approaches is that they do not need to track all the intermediate entities, and that they can use the nearest neighbor search \cite{indyk1998approximate} in the embedding space to quickly discover answers. 


\begin{table}[]
\centering
\caption{Prominent examples of \tnorms~and the corresponding \tnorms~when using the canonical negator $c(x)=1-x$.}
\begin{tabular}{llcl}
\toprule
\multicolumn{2}{c}{\tnorm} & negator & \tconorm  \\
\cmidrule(lr){1-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} 

% min
minimum (\godel) & $t(a,b)=\min(a,b)$
& \multirow{3}{*}{$c(x)=1-x$}
&  $s(a,b)=\max(a,b)$\\

% product
product & $t(a,b)=ab$
& & $s(a,b)=a+b-ab$ \\

% Luka
\luka & $t(a,b)=\max(x+y-1, 0)$
& & $s(a,b)=\min(x+y, 1)$ \\

\bottomrule
\end{tabular}

\label{tab:tnorms}
\end{table}
